An Ontology of Dark Patterns Knowledge: Foundations, Definitions, and a Pathway for Shared Knowledge-Building

Deceptive and coercive design practices are increasingly used by companies to extract profit, harvest data, and limit consumer choice. Dark patterns represent the most common contemporary amalgamation of these problematic practices, connecting designers, technologists, scholars, regulators, and legal professionals in transdisciplinary dialogue. However, a lack of universally accepted definitions across the academic, legislative and regulatory space has likely limited the impact that scholarship on dark patterns might have in supporting sanctions and evolved design practices. In this paper, we seek to support the development of a shared language of dark patterns, harmonizing ten existing regulatory and academic taxonomies of dark patterns and proposing a three-level ontology with standardized definitions for 65 synthesized dark patterns types across low-, meso-, and high-level patterns. We illustrate how this ontology can support translational research and regulatory action, including pathways to extend our initial types through new empirical work and map across application domains.

==> edpb-gl.tex <==

\section{Mapping EDPB guidelines definitions of dark patterns}

\NB{Liguri does not provide definitions of categories, so we only cite definitions of categories of Gray 2018. For DPs, we find related DPs in Liguri and Gray definitions.}

\subsection{Overloading}

{\bf EDPB definition:} "Overloading means users are confronted with an avalanche/large quantity of requests,
information, options or possibilities in order to prompt them to share more data or
unintentionally allow personal data processing against the expectations of the data subject."
%The following three dark pattern types fall into this category: Continuous prompting, Privacy Maze and Too Many Options

Conclusion: By nature, this category relates to both "Obstruction" and "Interface Interference". It relates to Interface Interference when it's about presenting information, like in Too Many Options. 
%
It also relates to Obstruction because Privacy Maze  prevents user to find the needed information or control. However, Privacy Maze is put in Hindering in EDPB GL because it presents user with too many steps. 

\CS{Looks like high level category of II}

\NB{EDPB seems to prefer to keep its original definition because it's more descriptive, but to mention "Nagging" means the same mechanism. However, EDPB does not cite any particular researchers in order not to single out anyone else.}

\subsubsection{Continuous prompting}

Below two definitions are presented.

\textbf{EDPB definition}
"Pushing users to provide more personal data than necessary for the purpose of processing or agree with another use of their data by repeatedly asking users to provide data or to consent to a new purpose of processing and offering arguments why they should provide it. Users are likely to end up giving in, wearied from having to refuse the request each time they use the platform, disrupting them in their use."

\textbf{Gray 2018 definition: Nagging}
"We define nagging as a minor redirection of expected functionality
that may persist over one or more interactions. Nagging
often manifests as a repeated intrusion during normal interaction,
where the user’s desired task is interrupted one or more
times by other tasks not directly related to the one the user is
focusing on."



Conclusion: Continuous Prompting is about one kind of requests that is repeated several times, while Nagging is more general that is interrupting the normal user activity one or more times.  

\NB{TODO: Discuss this with lead rapporteur: mechanism-wise, Continuous prompting uses the same mechanism as Nagging but it has a context-specific goal in data protection. We propose to rename it to Nagging underlying that we require several repetitions of a request.}

\CS{"Continuous P" = the high-level of Nagging, note (homogeneous requests, not heterog. are there downstream level types of N cross contexts? for now we never seen them}

\subsubsection{Privacy Maze}  

Below the definitions are presented.

\textbf{EDPB definition}
"When users wish to obtain certain information or use a specific control or exercise a data subject right, it is particularly difficult for them to find it as they have to navigate through too many pages in order to obtain the relevant information or control, without having a comprehensive and exhaustive overview available. Users are likely to give up or miss the relevant information or control." \\

Reflection: The difference with Dead End is that the path to information or control exists, but it is too hard to find, while in Dead End there is no path to the desired information or control.

\NB{We do not find a similar definition in the previous definitions of dark patterns.}

\NB{Interface Interference is about the one screen, while this pattern is about the user journey. So this doesn't seem to be a part of Interface Interference.}

\NB{We should verify the above statement with Colin.}

\CS{Inside of "Obstruction". How diff is from "Longer than Necessary"?}

\EH{Longer than Necessary has a comparative element (like reject on 2nd layer vs accept on 1st layer in a cookie banner). Privacy maze does not have a comparative element and it's about the journey in an interface.}

\EH{Privacy maze can be a meso-category of Obstruction}

\CS{"Overloading" and "Hindering" have common elements of Obstruction. Adding Overloading inside o Hindering}

\subsubsection{Too Many Options} Definitions are presented below. 


\textbf{EDPB definition:}
"Providing users with (too) many options to choose from. The amount of choices leaves users
unable to make any choice or make them overlook some settings, especially if information is
not available. It can lead them to finally give up or miss the settings of their data protection
preferences or rights.

\NB{We do not find a similar definition in the previous definitions of dark patterns. Nevertheless, it is definitely an instance of Interface Interference category because many options is a part of a design of the interface.}

\CS{Agree, inside Interface Interference. Maps to Meso category = with CMA: Information Overload, and Info Overload and Decoys; the name is quite literal, but Information Overload has been used in literature longer}


\subsection{Skipping}

{\bf EDPB definition:} "Skipping means designing the interface or user experience in a way that users forget or do not think about all or some of the data protection aspects." 
%The following two dark pattern types fall into this category: Deceptive Snugness and Look over there

{\bf Gray et al. 2018: Interface Interference}
"We define interface interference as any manipulation of the
user interface that privileges specific actions over others,
thereby confusing the user or limiting discoverability of important
action possibilities."

Skipping ensures that users get distracted by the interface and forget what they wanted to do. This corresponds perfectly to the Interface Interference category that uses interface to privilege specific actions and confuse the user.

\CS{we see Skipping under high-level "Sneaking", not II. The interface is designed for users to forget, because the info is presented in a way to be hidden to the user (?). Also, as it is high level category, wouldn't it make sense to adopt a more consensual naming?}

\NB{Proposal: see in "Fickle" -- OK!}

\subsubsection{Deceptive snugness}
Definitions below. 

\textbf{EDPB definition: }
"By default, the most data invasive features and options are enabled. Relying on the default
effect which nudges individuals to keep a pre-selected option, users are unlikely to change this
even if given the possibility."

\textbf{Gray et al. 2018 definition: Preselection}
"We define preselection as any situation where an option is
selected by default prior to user interaction. Preselection usually
manifests as a default choice that the shareholder of the
product wishes the user to choose; however, this choice is
often against the user’s interests or may provide unintended
consequences."

Conclusion: Deceptive snugness perfectly matches the Preselection definition. 

\NB{Rename it to Preselection because it's selected by default - OK! It's also easier to translate to other languages}

\CS{Agree with the mapping. it is also quite known as "Defaults" in the literature, but in DPLaw we call preselection} 

\subsubsection{Look over there}
Parallel definitions are presented below. 

\textbf{EDPB definition}

"A data protection related action or information is put in competition with another element which can either be related to data protection or not. When users choose this distracting option, they are likely to forget about the other, even if it was their primary intent."

\NB{To draw a difference from Hidden In Plain Sight, which is about the elements of the same nature, we propose the following change to make sure this definition is about elements of a different nature.}

\textbf{Proposal to change the EDPB definition}
"A data protection related action or information is put in competition with another element \em{which is not of the same nature but can be related to data protection}. When users choose this distracting option, they are likely to forget about the other, even if it was their primary intent."\\

\textbf{Gray 2018 definition of Aesthetic Manipulation}
"Aesthetic manipulation is any manipulation of the user interface that deals more directly with form than function. This
includes design choices that focus the user’s attention on one
thing to distract them from or convince them of something
else (e.g., Brignull’s "Misdirection")."


\textbf{Brignull's Misdirection}:
"The design purposefully focuses your attention on one thing in order to distract your attention from another."\\

\CS{yes, mappable to "False Hierarchy". Is there a need to make it as an autonomous category? Is the name intuitive?}

Conclusion: This dark pattern relates both to: i)  Misdirection-- if the competition is about visual representation; 
ii) False Hierarchy: if the competition is about the structure or order (part of II). 
Look Over There can be done with both Misdirection and False Hierarchy.




\subsection{Stirring}

{\bf EDPB definition:} "Stirring affects the choice users would make by appealing to their emotions or using visual nudges."
%The following two dark pattern types fall into this category: Emotional Steering and Hidden in plain sight

\textbf{Gray 2018 definition of Aesthetic Manipulation}
"Aesthetic manipulation is any manipulation of the user interface that deals more directly with form than function. This
includes design choices that focus the user’s attention on one
thing to distract them from or convince them of something
else (e.g., Brignull’s "Misdirection")."

It seems to match very well the Stirring to Aesthetic Manipulation 
since it includes both emotional manipulation (Toying with Emotion) 
and via visual nudges (False Hierarchy).

\CS{Stirring is presented as a high-level category,  mappable to II, which includes Toying with Emotion, False Hierarchy. Why to use such Label of Stirring as a high level category?}



\subsubsection{Emotional Steering}
Definitions below

\textbf{EDPB definition: }
"Using wording or visuals in a way that confers the information to users in either a highly positive outlook, making users feel good or safe, or in a highly negative one, making users feel scared or guilty. Influencing the emotional state of users in such a way is likely to lead them to make an action that works against their data protection interests."

\NB{"visuals" seems to refer only to pictures in English, while EDPB means a broader scope}

\NB{Proposal to change the EDPB definition:}
"Using \em{language, style, color or other visual elements} in a way that confers the information to users in either a highly positive outlook, making users feel good or safe, or in a highly negative one, making users feel scared or guilty. Influencing the emotional state of users in such a way is likely to lead them to make an action that works against their data protection interests." 


\textbf{Gray 2018 definition: Toying With Emotion}
"Toying with emotion includes any use of language, style, color,
or other similar elements to evoke an emotion in order to persuade the user into a particular action. This can manifest as cute or scary images, or as enticing or frightening language."

Conclusion: This DP matches exactly "Toying with Emotion". 

\NB{Our proposal to EDPB : to rename it to "Toying with emotion"}

\NB{EDPB tendency to keep the original definition}

\subsubsection{Hidden in Plain Sight}
Definitions are presented below. 

\textbf{EDPB definition:}
"Use a visual style for information or data protection controls that nudges users toward less
restrictive and thus more invasive options."

\textbf{Gray 2018: False hierarchy}
"False hierarchy gives one or more options visual or interactive precedence over others, particularly where items should be in parallel rather than hierarchical. This convinces the user to make a
selection that they feel is either the only option, or the best option."

\NB{This relates closely to False Hierarchy, but targets to hide more restrictive and protective options specifically.}

\EH{False Hierarchy is only a mechanism. Hidden in Plain Sight represents the goal as well but uses False Hierarchy to achieve the goal.}

\NB{Discuss the above observations with Colin.}

\CS{1) this label looks polemic - "Hidden in Plain Sight" guides a reader explicitly towards "hidden" information (as to the DP Hidden Info), 2) Looks like it has elements of "Privacy Zuckering" through all forms of nudges. My close to False Hierachy }

\subsection{Hindering}

{\bf EDPB definition:} "Hindering means obstructing or blocking users in their process of becoming informed or managing their data by making the action hard or impossible to achieve."
%The following three dark pattern types fall into this category: Dead end, Longer than necessary and Misleading information

{\bf Gray et al. 2018: Obstruction}
"We define obstruction as impeding a task flow, making an interaction more difficult than it inherently needs to be with the intent to dissuade an action. Obstruction often manifests as a major barrier to a particular task that the user may want to accomplish." \\

\EH{Should we call Nagging a meso level and it's to be included in Obstruction?
Why? Because Nagging has an idea  of blocking a user journey by impeding the user space and UX.
In other words, is Nagging a mechanism of implementing an Obstruction?
Nagging def. from Gray 2018 proposes a way to impede the task flow. Nagging is a mechanism only. Obstruction can contain Nagging as a mechanism with the goal to impede the user to make achieve their goal.}

\NB{Mechanism: impeding a task flow; goal: prevent the user from doing an action they wanted to do.}

Conclusion: Hindering corresponds very well to the Obstruction category since it is obstructing or blocking the users from making the action of their own choice and presents a barrier to a task the user wants to accomplish, such as being informed or manage their data.

\NB{Our proposal to rename "Hindering" to "Obstruction" in the EDPB GL.}

\CS{Looks like the high-level Obstruction. Why not to merge Overloading + Hindering altogether whith is subtypes?}

\NB{EDPB is ok renaming Hindering to Obstruction}

\subsubsection{Dead end}
Definitions are presented below. 


{\bf EDPB definition: }
"While users are looking for information or a control, they end up not finding it as a redirection link is either not working or not available at all. Users are left unable to achieve that task."

\NB{We do not find a similar definition in the previous definitions of dark patterns. Nevertheless, it is definitely an instance of Obstruction category. This is quite specific for Data Protection context where users search for GDPR-related information or control.}

\CS{See Brignul's "Roach Motel" inside Obstruction: The design makes it very easy for you to get into a certain situation (eg finding a link, control), but then makes it hard for you to "get out of it" (e.g. a subscription, accessing the info inside of that link ). the effect is that users are left unable to achieve that task}

\NB{We have discussed it with Estelle:  "dead end" is not about having a problem getting out once you've got in a certain situation. It's about searching for information or control, following intuitive path in the interface and being stuck in the end without finding the searched info or control.}

\subsubsection{Longer than necessary} 
Definitions below.

\textbf{EDPB definition:}
When users try to activate a control related to data protection, the user experience is made in a way that requires more steps from users, than the number of steps necessary for the activation of data invasive options. This is likely to discourage them from activating such control.

\NB{We do not find a similar definition in the previous definitions of dark patterns. Nevertheless, it is definitely an instance of "Obstruction" category.
This is about the time it takes for a user. It seems related to "Urgency" category because it is about the time: but in case of "Longer than Necessary" it's about the time takes to do something; while in the existing DPs of Urgency category (Countdown and Limited time) it's about creating the sense of urgency by using elapsed time as a mechanism. 
Conclusion: we don't think it's possible to group this together with DPs from Urgency category even though it's about time.}


\CS{Agree, mappable to the high category of Obstruction (and roach motel) in terms of time and UX. How is this different from Privacy Maze?}

\subsubsection{Misleading information}
Definitions below:

\textbf{EDPB definition:}
"A discrepancy between information and actions available to users nudges them to do something they do not intend to. The difference between what users expect and what they get is likely to discourage them from going further."

\textbf{Brignull definition of "Bait and Switch" from \url{https://www.deceptive.design/types}:}
"You set out to do one thing, but a different, undesirable thing happens instead."

\textbf{Gray 2018 describes "Bait and Switch" as}:
"Brignull’s "Bait and Switch" pattern makes it apparent that a
certain action will cause a certain result, only to have it cause a
different, likely undesired result." \\

Conclusion: This dark pattern relates very closely to "Bait and Switch". 
Because of the effect that users do not get what  they expect, this dark pattern seem to relate to the category of "Sneaking".
%
However, in Data Protection context, "Misleading information" is about 
the user trying to get certain control over her data and something 
else happens instead - generally, the user doesn't get the control she 
wanted to get. In "Sneaking", (see Gray 2018 for citation of text)
it's about an information that users would object to if they knew it. 
In Data Protection, it's about more actions than just objecting. 
Therefore, we do not believe that this DP is related to Sneaking category.

\NB{Proposal to EDPB to rename it to "Bait and Switch" because the original definition of Brignull matches perfectly. 
MI sounds static and doesn't represent the mismatch between the available information and the action available. Though "Bait and Switch" may not be selected by EDPB. Another name could be "Spoofing", Sham, Pretense, Mask, Veil, Disguise }

\CS{1) reading you now, i agree. @Colin, can we discuss the new category under II? 2) The fact that is says "Misleading Info", but then it refers to both controls+info, makes this name of this label confusing with other labels, eg with "Ambiguous Wording of Information"}

\CS{I stopped here}

\NB{EDPB agrees this needs changing yet noone knows how to call it exactly}

\subsection{Fickle}
Definitions below.

{\bf EDPB definition: Fickle} "The design of the interface is inconsistent and not clear, making it hard for users to navigate the different data protection control tools and to understand the purpose of the processing."

\EH{Fickle is about not matching what users want or expect. Differently from Misleading Info:   Fickle is about the place where info is supposed to be, but MI is about actions.}

\NB{TODO: The definition in the introduction of GL is not identical to the definition of Fickle in the appendix of GL - to fix}


{\bf Gray et al. 2018: Interface Interference}
"We define interface interference as any manipulation of the user  interface  that  privileges  specific  actions  over  others, thereby confusing the user or limiting discoverability of important action possibilities"

Conclusion: Fickle is a subgroup of \emph{Interface Interference} because it makes the interface inconsistent and unclear, however it does not push for specific actions over others, but rather confuses the user because the interface is inconsistent and unclear. For example, II contains Aesthetitc manipulation or Preselection which are not part of Fickle.

\NB{To me it seams that both "Fickle" and "Skipping" are specific instances of a wide category of "Interface Interference". Discuss with EDPB: does it make sense to add this observation to the GL?} 


%------------------------------------------------------
\subsubsection{Lacking hierarchy}

{\bf EDPB definition: Lacking hierarchy} "Information  related  to  data  protection  lacks  hierarchy,  making  information  appear  several times and being presented in several ways. Users are likely to be confused by this redundancy and to be left unable to fully understand how their data are processed and how to exercise control over them."

\EH{Idea for a new definition of "Lacking hierarchy" to make it clearly different from others, such as Privacy Maze and Conflicting information.}
Data protection information/control or the way to access them are structured in an inconsistent way, creating confusion for users and making it difficult for them to find an information or control.

\NB{We propose to EDPB to change the definition because it was too similar to Privacy Maze or Conflicting information. To make it more concrete, we have re-analyzed examples in the GL that relate to Lacking hierarchy and together came up with a new definition.}



We explain the differences between Privazy Maze (PM), Lacking hierarchy (LH) and Conflicting information (CI):
\begin{itemize}
\item  Privacy Maze = too long and complex path to an information or control, however the path exists (in Dead End it doesn't)
\item  Conflicting information = redundant information that creates confusion
\item  Lacking Hierarchy = ways of structuring information/controls or ways of accessing information/control that are inconsistent 
\end{itemize}


We copy here examples from EDPB GL to discuss:
\begin{itemize}
\item LH, Example 13: Information related to data subject rights is spread across the privacy notice. Although different data subject rights are explained in the section “Your options”, the right to lodge a complaint and the exact contact address is stated only after several sections \emph{and layers} referring to different topics. The privacy notice therefore partly leaves out contact details at stages where this would be desirable and advisable.
\NB{Proposal: remove "and layers" because it refers to the Privacy Maze. Without layers this example clearly demonstrates LH.}
\item LH, Example 14: The privacy policy is not divided into different sections with headlines and content. There are more than 70 pages provided. However, there is no navigation menu on the side or the top to allow users to easily access the section they are looking for. The explanation of the self-created term “creation data” is contained in a footnote on page 67.
\item LH, Example 38
\item LH, Example 49: The social media platform offers different versions (desktop, app, mobile browser). In each version, the settings (leading to access/objection etc.) are displayed with a different symbol, leaving users who switch between versions confused.

\end{itemize}

\NB{Propose to split into 2 DPs: 
(1) \emph{Lacking hierarchy}: redundancy of information and structure of information that wouldn't make it easy to read and find information (e.g. in a privacy notice). Ex. 13 is good demonstration (lodge complaint is in a different place than contact address) -- this should be put in "Left in the dark" because it's about the information only and not about the actions in the interface;
(2) \emph{Inconsistent interface}: interface isn't consistent across the social network -- in different contexts (across setting pages, across diff. devices (mobile vs. desktop) and how this difference impacts control and access to information. Ex. 38 gives ways to set preferences, but the order is reversed and can push people to make a less privacy-friendly choice.
}


{\bf Gray et al. 2018: False hierarchy} "False hierarchy gives one or more options visual or interactive precedence over others, particularly where items should be in parallel rather than hierarchical.  This convinces the user to make a selection that they feel is either the only option, or the best option."

{\bf Liguri 2021: Hidden information/aesthetic manipulation}
"Important information visually obscured"

\NB{New Inconsistent interface doesn't seem to be within Interface Interference category. We don't see existing patterns that are similar.
False Hierarchy is related to "hidden in plain sight" , it's not related to new LH because in new LH there is no hierarchy.}

%------------------------------------------------------
\subsubsection{Decontextualizing}

{\bf EDPB definition: Decontextualizing} "A data protection information or control is located on a page that is out of context. Users are unlikely  to  find  the  information  or  control  as  it  would  not  be  intuitive  to  look  for  it  on  this specific page."


Main concepts from EDPB examples: 
Option to delete data is located on an unrelated (out of context) tab or page. 

{\bf Gray  et al. 2018: Hidden information} 
"We define hidden information as options or actions relevant to the user but not made immediately or readily accessible. Hidden information may manifest as options or content hidden in fine print, discolored text, or a product’s terms and conditions statement. The primary motivator behind hidden information is the disguising of relevant information as irrelevant."

\NB{Double check that all the other newer paper refer to the same definiion of Gray 2018. We think it is (based on Miro) and so we compare only to the original definition of Gray 2018.}

\EH{D is very different from HI because D is about "what you're looking for is not in a place where you expect it to be (examples EDPB show info located under an unrelated page or under unrelated button).
HI is about visually less visible (disguising relevant info).}
	
{\bf Gray et al. 2018: Obstruction}
"We define obstruction as impeding a task flow, making an interaction more difficult than it inherently needs to be with the intent to dissuade an action. Obstruction often manifests as a major barrier to a particular task that the user may want to accomplish."

\EH{Globally, there are 2 tactics: either obstruct the user (make actions harder) or you make smth easier (nudging the user). }

\NB{Yes! These are 2 high-level mechanisms that are further used for different goals with sub-mechanisms that are more detailed.}

%{\bf Mathur: Hard to cancel} TO ADD - IT SEEMS TO CORRESPOND 

%{\bf Liguri: Immortal accounts} "Account and consumer info cannot be deleted"

{\bf Liguri: Hidden information/aesthetic manipulation}
"Important information visually obscured"

{\bf Notes:} 
At a low-level, it is an instance of \emph{hidden information} of Gray because it's a specific way to hide data protection information on pages that are out of context. It also correspond to \emph{Hidden information/aesthetic manipulation} of Liguri for the same reason.
In this way, decontextualising corresponds to the \emph{interface interference} category.

 
\subsection{Left in the dark}

{\bf EDPB definition:} "Left in the dark means an interface is designed in a way to hide information or data protection control tools or to leave users unsure of how their data is processed and what kind of control they might have over it regarding the exercise of their rights."
% The following three dark pattern types fall into this category: Language discontinuity, Conflicting information and Ambiguous wording or information.

\textbf{Gray 2018 definition: Hidden information}
"We define hidden information as options or actions relevant to
the user but not made immediately or readily accessible. Hidden
information may manifest as options or content hidden in
fine print, discolored text, or a product’s terms and conditions
statement. The primary motivator behind hidden information
is the disguising of relevant information as irrelevant."

In data protection context, the goal of LIND is to "leave users unsure of how their data is processed or how to control it", in HI the goal is more general - that is make information or actions harder to access. We conclude that LIND goal is more specific than HI and also includes a goal to "leave users unsure".

\NB{We may want to make sure we have a category for hiding information and another one for confusing the user? So far they are somehow both mixed in "Fickle" and "Left in the dark"}

\subsubsection{Language discontinuity}

\textbf{EDPB definition: }
"Information related to data protection is not provided in the official language(s) of the country
where users live, whereas the service is. If users do not master the language in which data
protection information is given, they will not be able to easily read it and therefore likely to
not be aware of how data are processed."

This definition is very specific to the language and did not appear before in the dark patterns classifications.

\NB{We propose to EDPB to move it to "Fickle" category where  
the interface is inconsistent and not clear, making it hard for users to navigate. }


\subsubsection{Conflicting information} 

\textbf{EDPB definition:}
"Giving pieces of information to users that conflict with each other in some way. Users are likely
to be left unsure of what they should do and about the consequences of their actions,
therefore likely not to take any and to just keep the default settings."

Information can be either textual or visual, like in Example 26, where information is communicated vie the colors of toggles.
This dark pattern does not seem to match any existing one. 


\subsubsection{Ambiguous wording or information}

\textbf{EDPB definition:}
"Using ambiguous and vague terms when giving information to users. They are likely to be left
unsure of how data will be processed or how to exercise control over their personal data."

This dark pattern does not seem to match any existing one. 



==> edpbcomparison.tex <==
\begin{table*}
\caption{Mapping EDPB~\cite{EDPB2022} dark patterns to our ontology. }
\label{tab:regulatory}
\begin{tabularx}{\textwidth}{p{2cm}p{5cm}p{5cm}}
\hline
& EDPB dark pattern type & Our ontology type \\
\hline
\multirow{5}{2cm}{Mapping high-level dark patterns} % (when both EDPB and our mapping are high level)
&    Overloading & Interface Interference \\ 
&    Stirring & Interface Interference \\ 
&    Fickle & Interface Interference \\ 
&    Skipping & Sneaking \\ 
&    Obstructing & Obstruction \\ 
\hline
\multirow{13}{2cm}{Mapping low- and meso-level dark patterns}
&    Continuous prompting  &  Nagging \\
&     Decontextualising.  &  Information without Context \\
&     Lacking hierarchy  &  False hierarchy \\
&     Too many options  &  Choice overload \\
&      Deceptive snugness  &  Privacy-invesive defaults \\
&     Look over there  &  Visual prominence \\
&     Emotional Steering  &  Positive or negative framing \\
&     Hidden in plain sight  &  Hidden information \\
&     Misleading action  &  Feedforward ambiguity \\
&     Language discontinuity  &  Wrong Language \\
&     Left in the dark  &  Hidden information \\
&     Inconsistent interface  &  not mapped \\ 
&     Longer than necessary  &  not mapped \\ 
\hline     
\end{tabularx}
\end{table*}

==> evolution-stripped.tex <==
\textless ccs2012\textgreater{} \textless concept\textgreater{}
\textless concept\_id\textgreater10003120.10003121\textless/concept\_id\textgreater{}
\textless concept\_desc\textgreater Human-centered computing~Human
computer interaction (HCI)\textless/concept\_desc\textgreater{}
\textless concept\_significance\textgreater500\textless/concept\_significance\textgreater{}
\textless/concept\textgreater{} \textless concept\textgreater{}
\textless concept\_id\textgreater10003120.10003121.10011748\textless/concept\_id\textgreater{}
\textless concept\_desc\textgreater Human-centered computing~Empirical
studies in HCI\textless/concept\_desc\textgreater{}
\textless concept\_significance\textgreater500\textless/concept\_significance\textgreater{}
\textless/concept\textgreater{} \textless/ccs2012\textgreater{}

\section{Introduction}\label{introduction}

Deceptive design practices are increasingly common in digital
environments, impacting digital experiences on social
media~\cite{Schaffner2022-nn,Mildner2021-kp},
e-commerce~\cite{Mathur2019-hx}, mobile devices~\cite{Gunawan2021-pr},
cookie consent banners~\cite{Gray2021-zf}, and
gaming~\cite{Zagal2013-gj}, among others. An increasingly dominant
framing of these deceptive practices is known as ``dark
patterns''\footnote{We use this term to connect our efforts to prior
  scholarship and legal statute, recognizing that other terms such as
  ``deceptive design'' or ``manipulative design'' are sometimes used to
  describe similar tactics. While the ACM Diversity and Inclusion
  Council has included dark patterns on a
  \hyperref[https:ux2fux2fwww.acm.orgux2fdiversity-inclusionux2fwords-matter]{list
  of potentially problematic terms}, there is no other term currently in
  use that describes the broad remit of dark patterns practices that
  include deceptive, manipulative, and coercive patterns that limit user
  agency and are often hidden to the user.}---describing instances where
design choices subvert, impair, or distort the ability of a user to make
autonomous and informed choices in relation to digital systems
regardless of the designer's intent~\cite{CPRA,DSA2022,FTC2022}.

While the origins of dark patterns as a concept to describe manipulative
design practices goes back over a decade to when the term was coined by
practitioner and scholar Harry Brignull~\cite{Brignull_undated-vj}, in
the past five years there has been growing momentum in the use of the
term to unite scholars, regulators, and designers in transdisciplinary
dialogue to identify problematic practices and find ways to prevent or
discourage the use of these patterns. According to a recent study of the
historical evolution of \#darkpatterns on Twitter by Obi and
colleagues~\cite{Obi2022-bd}, since 2019, conversations have included
stakeholders not only from design and technology but also social
scientists, lawyers, journalists, lawmakers, and members of regulatory
bodies and consumer protection organizations.

Within the regulatory space, in 2022 alone, the term ``dark patterns''
was codified into EU law in the Digital Services Act~\cite{DSA2022}, the
Digital Markets Act~\cite{DMA}, and the Data Act
proposal~\cite{Data-Act-proposal}, and into US law in the California
CPRA~\cite{CPRA}. Regulatory bodies such as the US Federal Trade
Commission (FTC), the UK Competition and Market Authority (CMA), the EU
Commission, the European Data Protection Board (EDPB) and the the
Organisation for Economic Co-operation and Development (OECD) have
released guidance on specific types of dark patterns with various levels
of overlap with definitions from academic
scholarship~\cite{EDPB2022,CMA2022,EUCOM2022,FTC2022, Oecd2022}. In late
Summer 2023, the Department of Consumer Affairs in India also released
draft guidelines regarding dark patterns~\cite{india_2023-ek}. In
addition, the concept of dark patterns has been leveraged in sanctions
against companies that have relied upon manipulative practices. Recent
actions include a \$245 million USD judgment against Fortnite, a product
from Epic Games, for their use of manipulative practices to encourage
the purchase of content~\cite{Wodinsky2022-bj} and multiple settlements
by various US states against Google for their use of dark patterns to
obtain location data~\cite{Press_Release2022-fq,Weatherbed2022-oj}. In
the EU, both Data Protection Authorities (DPAs) and court decisions have
forbidden certain practices related to dark patterns, including:
pre-selection of choices~\cite{CJEU-Planet49-19}; refusing consent if it
is more difficult than giving
it~\cite{CNILvsGoogle2021,CNILvsFacebook2022}; and misinforming users on
the purposes of processing data and how to reject
them~\cite{CNILvsFacebook2022, LuxDPA-amazon}.

As part of this convergent discourse, HCI scholars have addressed the
threat of dark patterns in a wide range of publications, proposing
definitions and types of dark
patterns~\cite{Bosch2016-vc,Gray2018-or,Mathur2019-hx,Mathur2021-rc,Luguri2021-bg}.
However, the specific forms that dark patterns can take, the role of
context, the ubiquity of the practices, the technologies used or
application area, the comparative harms of different patterns, remedies,
and the role of user education and countermeasures are still a topic of
ongoing research. The consequence of this dynamic topic is of an
ever-expanding list of categories and variants whose scale continues to
grow.

Two large challenges face an ongoing transdisciplinary engagement with
the concept of dark patterns. First, the literature has grown quickly
and is siloed, often lacking accurate citation provenance trails of
given typologies and definitions, making it difficult to trace where new
or more detailed types of patterns emerged and under which conditions.
The space that dark patterns scholars have sought to cover is also vast,
with important research occurring in specific domains (e.g., games,
e-commerce, privacy and data protection) and across different
technologies and modalities (e.g., mobile, desktop, conversational user
interfaces (CUIs), AR/VR), as shown in a recent systematic review of
dark patterns literature~\cite{Gray2023-systematic}. This diversity of
research has led some scholars to propose fragmentary, domain-specific
typologies without necessarily finding commonalities across domains.
Second, regulators---the ultimate decision makers that could provide
legal certainty to this landscape--- and policy makers have been
interested in the scholarly conversation regarding dark patterns, but
have in some cases created wholly new domain-related terminology to
describe types already known in the academic literature
(e.g.,~\cite{EDPB2023}. In other cases, regulators and policymakers have
inconsistently cited academic sources (e.g.,~\cite{FTC2022,EDPB2023})
making connections across the regulatory, legal, and academic spaces
fraught.

We seek to support these challenges and ongoing conversations by
building the foundation for a common ontology of dark patterns. By
taking the first steps towards building an ontology, we seek to create a
shareable, extendable, and reusable knowledge representation of dark
patterns. This groundwork for an ontology is both domain and application
agnostic though it has potential utility in domain or context-specific
instances as well. For instance, the {\emph{Bad Defaults}} dark pattern
is often embedded in settings menus, pre-set so that users share
personal information on social media platforms or accepting to receive
advertising content on online shopping sites unknowingly. Such
context-specific instances are enabled through {\emph{Interface
Interference}}---a domain-agnostic strategy used to manipulate
interfaces, privileging certain actions and, thus, limiting
discoverability of alternatives. As noted by
Fonseca~\cite{Fonseca2007-mv}, ontologies can be useful in supporting
social science research by ``creating better conceptual schemas and
applications.'' To create this preliminary ontology, we build upon ten
contemporary taxonomies of dark patterns from both the academic and
regulatory literature, and thereafter we identify three levels of
hierarchy for pattern types. Hence we harmonize concepts across these
taxonomies to provide a consistent and consolidated, shared, and
reusable dark patterns ontology for future research, regulatory action,
and sanctions.

We make four contributions in this paper. First, we introduce the
hierarchical concepts of low-level, meso-level, and high-level dark
patterns to the literature, disambiguating UI-level patterns that may
lead to opportunities for detection (low-level) and strategies that may
be targeted by policy and legislation (meso- and high-level). Second, by
analysing the provenance of dark patterns from academic and regulatory
sources, we identify when patterns first emerged and how naming has
evolved over time and across sources. Third, we describe a common
definition syntax, set of definitions, and hierarchy of dark patterns
that aligns disparate terminology from scholars and regulators. Fourth,
we demonstrate how the ontology can be strengthened and extended through
additional empirical work, and how the ontology can effectively be
utilized by practitioners, scholars, regulators, and legal professionals
to support transdisciplinary action.

\section{Motivation \& Background}\label{motivation-background}

Since the initial set of a dozen types of dark patterns proposed by
Brignull in the 2010s, research has focused on related issues from
multiple angles including, but not limited to, e-commerce, games, social
media, and IoT~\cite{Gray2023-systematic}. While this scholarship
contributes significant insights to the discourse, we noticed varying
approaches to adopt existing descriptions, defining novel scenarios in
which users are harmed. Meanwhile, the specification of individual
typologies creates a certain ambiguity within the overall discourse on
the matter. In developing this ontology, we confront numerous timely
issues relating to the description of dark patterns, the study of dark
patterns and their harms through empirical work, and the leveraging of
this scholarship to support legal and regulatory action.

Dark patterns are known to be ubiquitous; however, most pattern types
have been explored in relatively narrow contexts or domains with more
scholarship needed to fully define causal links, harms, and impacted
populations~\cite{Gray2023-systematic}. The HCI community has been
engaged and interested in impacting society and the future of technology
practices relating to dark
patterns~\cite{Gray2023-SIG,Lukoff2021-fk}---and indeed, HCI scholars
have been central in the study of dark patterns, revealing insights
relating to the harm and severity of dark patterns that then support
enforcement action and regulation. However, we currently lack a shared
landscape of definitions, types, and language to unify the study of dark
patterns. Without this shared landscape, research has become (and will
continuously be) fragmented by domain, context, and technology
type---which if not addressed, may lead to duplicated effort by scholars
working on similar issues in different domains, and additionally may
hamper regulatory enforcement due to lack of precision and shared
language regarding precisely what dark patterns are used and with what
effect. Such lack of a shared ontological framework may also restrict
traceability and searchability of dark patterns.

Our work unifies practitioner, scholarly, and regulatory efforts that
describe the range of dark patterns, leading to a shared vocabulary and
ontology that allows for coordination of efforts across diverse contexts
(e.g., technologies, specific functionality, areas of technology use)
and stakeholders (e.g., regulators, legal scholars, social scientists,
practitioners). This ontology will support not only the advancement of
scholarship, but also translational and transdisciplinary efforts that
connect scholarship to legal sanctions and regulatory frameworks. For
instance, there are now high-level prohibitions of dark patterns by
regulatory authorities and legal statute; however, the specific
low-level practices that should be deemed illegal under these
prohibitions are not yet detailed in enforcement action or case law.
This paper connects these different strands of work by harmonizing
regulatory and academic work into a single ontology, enabling future
scholars from all disciplines to utilise our structures and definitions
to support their work.

\section{Methodology}\label{methodology}

We used a qualitative content analysis approach~\cite{Hsieh2005-ld} to
identify and characterize elements of existing dark patterns taxonomies
using the method described in
Figure~\hyperref[fig:ontologymethod]{{[}fig:ontologymethod{]}}.

As a research team, we leveraged our collective experiences in
human-computer interaction, design, computer science, law, and
regulation. Specifically, our team included established dark patterns
scholars, including one with a focus on human-computer interaction and
design (Authors 1 and 4), one with a focus on computer science and web
measurement and experience in regulation (Author 3), and one with a
background in computer science and data protection law (Author 2).
Across these perspectives, in accordance with previous scholarship, we
sought to characterize dark patterns in a transdisciplinary way, drawing
on multiple disciplinary perspectives that provide differing views on
the origins and types of dark patterns~\cite{Gray2021-zf}. However,
these backgrounds also introduce gaps, tensions, and opportunities that
relate to the unique experience and academic training of each author. To
account for this difference in perspective, each dark pattern type was
initially reviewed by each author independently before engaging in
conversation amongst the researchers that led to the final agreement on
the harmonized type and definition.

\includegraphics{figures/ontology_method.pdf}

\phantomsection\label{fig:ontologymethod}{}

\subsection{Data Collection}\label{data-collection}

We collected dark patterns taxonomies from a total of 10 sources,
including:

\begin{enumerate}
\item
  A set of patterns shared on \url{https://darkpatterns.org} since 2010
  by Harry Brignull\footnote{This collection of dark patterns was moved
    to \url{https://www.deceptive.design} in 2022, but the 12 patterns
    we drew on have been stable since 2018 when the final pattern,
    ``confirmshaming,'' was added. In 2023, this website was updated to
    include additional pattern types, resulting in a modified collection
    of 16 types.}
\item
  Scholarly academic sources that present a distinct and comprehensive
  taxonomy and have either been cited in scholarly and regulatory
  literature supporting proposed taxonomies or where dark patterns types
  have been used in regulatory reports without citation but with similar
  or identical
  naming~\cite{Bosch2016-vc,Gray2018-or,Luguri2021-bg,Mathur2019-hx}.
\item
  Public reports from stakeholders and regulators in the EU, UK, and USA
  that include a dark patterns
  taxonomy~\cite{EDPB2022,EUCOM2022,CMA2022,FTC2022,Oecd2022}.
\end{enumerate}

The selection of these sources encompass, at the time of our data
collection in Fall 2022: i) the most commonly cited taxonomies in the
research literature that contributed to regulatory taxonomies in a
direct or indirect way, ii) the most comprehensive set of regulatory
literature, and iii) all taxonomies cited in regulatory reports,
demonstrating an implicit or direct translation from academia to
regulation and policy.

\subsection{Data Analysis}\label{sec:data-analysis}

Once we gathered the set of taxonomies, we began our analysis by
identifying the constitutive components of each taxonomy without
considering overlaps across sources through a bottom-up approach.

\textbf{Quantification of dark pattern types} Across the ten taxonomies
from academic and regulatory sources collected in Fall 2022, we
identified 186 low-level and 59 high-level patterns (a total of 245
patterns). After our initial analysis, the patterns used on Brignull's
site (\url{https://www.deceptive.design}) were substantially updated in
the Summer 2023, and we collected the additional set of patterns for
that source---resulting in 11 total sources. Also, the EDPB regulatory
report was made final in February 2023, and we used its final taxonomy
in this paper after completing our initial mapping in the Fall 2022
based on the draft report taxonomy. Based on the updates to the EDPB
guidelines and Brignull's site in the Spring and Summer 2023, the total
number of patterns we analyzed included 203 low-level (adding 1 new
pattern from the revised EDPB guidelines and 16 patterns from the
updated Brignull site) and 59 high-level patterns---\textbf{a total of
262 patterns} (see Tables~\hyperref[tab:academic]{{[}tab:academic{]}}
and \hyperref[tab:regulatory]{{[}tab:regulatory{]}} in the supplemental
material). All taxonomy elements are included in supplemental material
for other scholars to build upon.

\textbf{Rationale underlying the high number of dark pattern types} This
large number of discrete elements is perhaps unsurprising, since each
typology author has used a different point of focus and categorization
based on the sector they sought to describe or support. For instance,
Mathur et al.~\cite{Mathur2021-rc} and the CMA~\cite{CMA2022} focus on
e-commerce; the EDPB focuses on data protection practices within social
media platform interfaces~\cite{EDPB2022}, and the FTC~\cite{FTC2022}
and EU Commission~\cite{EUCOM2022} focus on guidance specific to their
jurisdictions and underlying legal authority. The types themselves also
evolved in one case due to input from the practitioner and regulatory
community, which is the case of the EDPB naming of patterns changed
slightly from the 2022 draft report to the final 2023 report, with one
high-level strategy ``hindering'' changing to ``obstructing'' to bring
it into better alignment with academic taxonomies.

\includegraphics{figures/ontology_miro.png}

\phantomsection\label{fig:ontologymiro}{}

\subsubsection{Creating the Ontology
Framework}\label{sec:ontologymethod}

We used the following procedure to carefully identify existing taxonomy
components, their source, relationships and similarities between
components across taxonomies, visualized in
Figure~\hyperref[fig:ontologymethod]{{[}fig:ontologymethod{]}}:

\begin{enumerate}
\item
  \textbf{Aggregating existing patterns.} We first listed all high- and
  low-level patterns verbatim in the structure originally indicated in
  the textual source. \emph{High-level patterns} include any instances
  where the pattern is denoted as a category, strategy, goal, intention,
  or other parent in a parent-child relationship. \emph{Low-level
  patterns} indicate specific patterns that are included as a child in a
  parent-child relationship, or are otherwise undifferentiated in
  hierarchy (e.g., Brignull's patterns).
\item
  \textbf{Identifying provenance through direct citations and
  inference.} Based on citations provided in the source-document, we
  indicated any instances where patterns were \emph{directly cited} or
  otherwise duplicated from previous sources. Because many patterns were
  uncited---particularly in regulatory reports---we also relied upon
  citations elsewhere in the document or explicit use of existing
  pattern vocabulary and definitions from previously published sources,
  which we indicate as \emph{inferential}. We used these direct and
  inferential citation patterns to identify where patterns were first
  introduced, even if they appeared alongside other patterns that had
  been published previously. This allowed us to map the historical
  progression of high- and low-level types over time.
\item
  \textbf{Clustering similar patterns.} We grouped patterns that
  appeared either to be identical or similar (in a \emph{is-a} or
  \emph{equivalent-to} relationship) on Miro (see
  Figure~\hyperref[fig:ontologymiro]{{[}fig:ontologymiro{]}}), using
  definitions to identify affinities among patterns that did not have
  identical names. This portion of the analysis was the most extensive,
  including in depth conversations between an HCI and legal scholars and
  a careful reading of the definitions as they might be understood by
  designers and lawyers. We tried out numerous different groupings based
  on what we understood to be the main focus of each pattern and then
  sought to characterize what level of pattern each represented.
\item
  \textbf{Creating meso-level patterns.} From the findings of this
  visually-organized analysis procedure, we recognized that there were
  not only low- and high-level patterns present, but also a
  \emph{``meso''} level of pattern knowledge. By recognizing
  similarities among low-level patterns, we introduced \emph{meso-level
  patterns} into our analysis, identifying these patterns by using the
  names or elements of existing taxonomies where possible, or coining
  new names to characterize the low-level patterns we grouped together.
  If the pattern cluster was specific to low-level UI concerns, we
  sought to identify a meso-level pattern name that was more abstract
  and could contain the low-level pattern. If the pattern represented a
  meso-level abstraction, we did not seek to identify specific low-level
  instantiations---instead leaving that task for future scholarship
  efforts in domain- and technology-specific areas.
\item
  \textbf{Finalizing the ontology.} Across these three levels of
  hierarchy, we grouped 233 of the 245 taxonomy elements\footnote{Four
    ungrouped elements were from the CMA report~\cite{CMA2022} in Fall
    2022 and described generic elements of digital systems which were
    not explicitly framed as deceptive or manipulative: Choice
    Structure, Choice Information, Feedback, and Messengers. All eight
    high-level patterns from Bösch~\cite{Bosch2016-vc} were also
    excluded since they were not reiterated in any downstream
    literature.}. After evaluating the changes to the EDPB guideline
  taxonomy and updated Brignull taxonomy in Spring and Summer 2023, we
  updated our mapping of 262 patterns, which resulted in no additional
  novel pattern types. The final ontology includes 5 high-level
  patterns, 25 meso-level patterns, and 35 low-level
  patterns---\textbf{a total of 65 patterns}.
\end{enumerate}

\subsubsection{Harmonizing Definitions of Dark Patterns
Types}\label{harmonizing-definitions-of-dark-patterns-types}

Building on this ontology framework, we then proceeded to create a
definitional syntax across the three levels of the ontology and then
created definitions for each final pattern using the following approach:

\begin{enumerate}
\item
  \textbf{Creating definition syntax.} We evaluated the range of
  approaches to definitions in the existing taxonomies.

  \begin{itemize}
  \item
    \emph{Short vs long definitions.} Some definitions were very short
    (e.g., the EU Commission's definition for \emph{forced
    registration}: ``Consumer tricked into thinking registration is
    necessary'') while other definitions were more elaborate (e.g., the
    FTC's definition for \emph{baseless countdown timer}: ``Creating
    pressure to buy immediately by showing a fake countdown clock that
    just goes away or resets when it times out. Example: `Offer ends in
    00:59:48'\,''; the EU Data Protection Board's definition for
    \emph{longer than necessary}: ``When users try to activate a control
    related to data protection, the user journey is made in a way that
    requires more steps from users, than the number of steps necessary
    for the activation of data invasive options. This is likely to
    discourage them from activating such control.'').
  \item
    \emph{Description of the definitions.} Most definitions were based
    in a description of user interaction with a system, like the
    examples above; however, Brignull's 2018 definitions were written in
    first-person language demonstrating how a user would experience a
    dark pattern (e.g., the definition for \emph{roach motel}: ``You get
    into a situation very easily, but then you find it is hard to get
    out of it (e.g. a premium subscription).'') Interestingly,
    Brignull's 2023 language appears to model other taxonomies with all
    definitions beginning with ``The user struggles...,'' ``The user
    expects...'' or similar structures.
  \item
    \emph{Definition structure and syntax.} We used an iterative process
    where two authors independently and collaboratively tested different
    definition structures. Based on these efforts and through
    discussion, we finalized sample definition structures and syntax
    that captured the relevant type of knowledge (e.g., strategy, angle
    of attack, means of execution). For instance, all high-level
    patterns included the interplay of an undesired action and a
    limitation of their decision-making or free choice. Meso-level
    patterns addressed a mismatch in users' expectations of a system and
    the relevant impact. Low-level patterns identified how they manifest
    their parent high- and meso-level pattern in relation to one or more
    elements of the UI and a mismatch of expectation and resulting
    effect on the user experience.
  \end{itemize}
\item
  \textbf{Creating and evaluating high- and meso-level pattern
  definitions.} We then drafted definitions for all high- and meso-level
  patterns, iterating on the structure until we found a syntax that
  appeared to address all critical elements of the existing definitions
  and allow us to clearly indicate how the pattern subverted user
  autonomy and manifest as deceptive or coercive. We began with
  definitions at these levels since low-level patterns were already
  grounded in specific UI examples, and thus more effort was needed to
  identify what components a definition at a higher level of abstraction
  should include. Regarding evaluation, our set of 30 definitions and
  the draft definition structures were then shared via an open Google
  Doc with members of a large Slack community focused on research and
  enforcement action relating to dark patterns. We asked this community
  for feedback on the utility of the definitions, the completeness of
  the definition structures, and the ability of these definitions to
  leave as open-ended the many different low-level manifestations of
  dark patterns. Multiple community members gave us feedback which
  allowed us to validate the general face validity of the definitions,
  and we continued to iterate on our structure and language in response.
\item
  \textbf{Finalizing low-level pattern definitions.} After mapping out
  the initial 30 definitions, we created definitions for the 34
  low-level patterns that were grounded in the specifics of the UI
  execution. These patterns were easier to write since many taxonomy
  definitions (in particular those from Brignull~\cite{Brignull_2023},
  Gray~\cite{Gray2018-or}, and the FTC~\cite{FTC2022}) included richer
  detail for patterns that pointed towards a real-world implementation.
  As a research team, we read and edited the definitions until we were
  satisfied with their level of consistency and relationships to the
  higher-level categories in which they belonged. All definitions are
  included in the appendix of this paper and supplemental materials to
  support future work.
\end{enumerate}

\section{Mapping the Evolution of Dark Patterns}\label{sec:evolution}

\includegraphics{figures/ontology_evolution_v1.1.png}

\phantomsection\label{fig:ontologyevolution}{}

Pattern names have largely stabilized in the past five years, including
high-level pattern types (e.g., nagging, obstruction, sneaking,
interface interference, forced action) and low-level patterns (including
Brignull's~\cite{Brignull_undated-vj,Brignull_2023} and those introduced
by Gray et al.~\cite{Gray2018-or} and Mathur et
al.~\cite{Mathur2019-hx}). A mapping of these patterns over time across
the academic and practitioner sources we considered is included in
Figure~\hyperref[fig:ontologyevolution]{{[}fig:ontologyevolution{]}}.

\textbf{High-level patterns} were most likely to co-occur across
multiple sources. For instance, Gray et al.'s~\cite{Gray2018-or}
original five high-level ``dark pattern strategies'' were found across
multiple other sources, even if they were not consistently cited:
nagging \cite{Luguri2021-bg,EUCOM2022}, obstruction
\cite{Mathur2019-hx,Luguri2021-bg,EUCOM2022,FTC2022}, sneaking
\cite{Mathur2019-hx,Luguri2021-bg,EUCOM2022,FTC2022}, interface
interference \cite{Luguri2021-bg,EUCOM2022,FTC2022}, and forced action
\cite{Mathur2019-hx,Luguri2021-bg,EUCOM2022,FTC2022} (FTC uses ``coerced
action'' instead). As shown in
Figure~\hyperref[fig:ontologyevolution]{{[}fig:ontologyevolution{]}},
virtually all of the high level patterns proposed by Gray et al. in 2018
were carried forward in other academic taxonomies. In Brignull's 2023
changes to \url{https://www.deceptive.design}, multiple high-level
strategies from Gray et al.'s~\cite{Gray2018-or} taxonomy were added to
the website (nagging, obstruction, sneaking, forced action, visual
interference)---however, these changes were not cited and Brignull
continued his practice of not providing direct citations or hierarchical
structure to his patterns. After their introduction in Mathur et
al.~\cite{Mathur2019-hx}, newly introduced categories relating to social
psychology or behavioral economics also became common: urgency
\cite{Luguri2021-bg,EUCOM2022,FTC2022}, scarcity
\cite{Luguri2021-bg,FTC2022}, and social proof
\cite{Luguri2021-bg,EUCOM2022,FTC2022} (the FTC bundles ``Endorsements''
with ``social proof''). We have grouped these types together as part of
a sixth high-level pattern of ``social engineering.''

\textbf{Domain or context-specific patterns.} The most volatility has
occurred in relation to \emph{domain-} or \emph{context-specific
patterns}. These include expansions of Mathur et
al.'s~\cite{Mathur2019-hx} high-level patterns of ``social proof'' and
``scarcity,'' which have since been reiterated by the EU
Commission~\cite{EUCOM2022} and OECD~\cite{Oecd2022} and extended by the
CMA~\cite{CMA2022} and FTC~\cite{FTC2022} taxonomies. In addition, the
EDPB guidance on dark patterns in social media~\cite{EDPB2022} included
a wholly new set of 6 high-level and 15 low-level patterns, although the
majority of these could be inferred as similar to already existing
patterns proposed in the academic literature. Importantly, though, the
EDPB taxonomy included multiple patterns which we found to be new
low-level or meso-level additions, including ``privacy maze,'' ``dead
end,'' ``conflicting information,'' ``information without context''
(which we renamed from the EDPB pattern ``decontextualizing''), and
``visual prominence'' (which we renamed from the EDPB pattern ``look
over there''). Similarly, the CMA taxonomy focused on choice
architecture as a guiding structure with three categories focused on
choice ``structure,'' ``information,'' and ``pressure.'' This taxonomy
structure also yielded new patterns, including ``bundling,'' ``complex
language,'' and ``personalization.''

Our analysis demonstrates the value in classifying or generating
context-specific patterns that illuminate gaps in current taxonomies,
and also the benefit of mapping these patterns within larger ontologies
to identify abstractions of patterns that may apply across many domains,
contexts, and legal fields. Our final ontology mapping is included in
Figures~\hyperref[fig:ontologypt1]{{[}fig:ontologypt1{]}} and
\hyperref[fig:ontologypt2]{{[}fig:ontologypt2{]}} and can also be found
in the supplementary materials.

\includegraphics{figures/Ontology_v1_01.pdf}

\phantomsection\label{fig:ontologypt1}{}

\includegraphics{figures/Ontology_v1_02.pdf}

\section{Creating a Definitional Structure by Ontology
Level}\label{creating-a-definitional-structure-by-ontology-level}

As described in Section~\hyperref[sec:ontologymethod]{3.2.1}, our
ontology includes three different levels of hierarchy:

\begin{itemize}
\item
  \textbf{High-level patterns} are the most abstracted form of
  knowledge, including general \emph{strategies} that characterize the
  inclusion of manipulative, coercive, or deceptive elements that might
  limit user autonomy and decision making. These patterns are
  context-agnostic and can be employed through a range of modalities and
  technologies (e.g., desktop, mobile, VUIs, VR/AR) and application
  types (e.g., e-commerce, gaming, social media).
\item
  \textbf{Meso-level patterns} bridge high- and low-level forms of
  knowledge and describe an \emph{angle of attack} or specific approach
  to limiting, impairing, or undermining the ability of the user to make
  autonomous and informed decisions or choices. These patterns are
  content-agnostic and may be interpreted in a contextually-appropriate
  way based on the specific context of use or application type.
\item
  \textbf{Low-level patterns} are the most situated and contextually
  dependent form of knowledge, including specific \emph{means of
  execution} that limits or undermines user autonomy and decision
  making, is described in visual and/or temporal form(s), and is likely
  to be detectable through algorithmic, manual, or other technical
  means.
\end{itemize}

To create a definitional structure for each level, we first used a
subset of approximately ten dark patterns types and definitions in order
to ``play-test'' a combined and unified definition for dark patterns
types at multiple levels of granularity (i.e., high, meso, low). Through
this process, we considered not only the level of abstraction inherent
in dark patterns at differing levels, but also the interaction between:
the user's expectations of what should or would be likely to occur
(i.e., manipulation of the gulf of execution); the user's identification
that something had occurred that they did not wish to happen (i.e.,
manipulation of the gulf of evaluation); and the mechanisms used to
inform or execute manipulation in either of these prior elements. We
also considered cases where the deception or manipulation was likely to
be hidden to the user (e.g., cases of sneaking, obstruction, or
interface interference) as well as cases where deception or coercion was
overt and known to the user (e.g., forced action). Based on this
iterative generation of a definitional structure, we created a
standardized syntax for each dark pattern level, described below. All 65
final definitions are included as a supplemental material.

\subsection{High-Level Patterns}\label{high-level-patterns}

\begin{quote}
\textbf{\{HIGH-LEVEL DARK PATTERN\}} is a strategy which
\textbf{\{UNDESIRED ACTION\}} that {[}optionally, if known to users,
would{]} \textbf{\{DISTORT/SUBVERT/IMPEDE/OTHERWISE LIMIT USERS'
AUTONOMY, DECISION-MAKING, OR FREE CHOICE\}}.
\end{quote}

Across our 5 high-level pattern definitions, we considered
{\emph{undesired actions}} such as: hiding, disguising, delaying,
redirecting, repeating, impeding, privileging, or requiring actions. We
also considered a range of \emph{mechanisms} that could be used to limit
users' autonomy, decision-making, or free choice such as: foregrounding
unrelated tasks, dissuading a user from taking an action, confusing the
user, limiting discoverability of action possibilities, causing a user
to unintentionally take an action they would likely object to, or
forcing a user to take an action they would not otherwise take. Most of
these definitions placed a focus on mechanisms which were primarily
hidden, resulting in the user being deceived, such as: ``\emph{Interface
Interference} is a strategy which privileges specific actions over
others through manipulation of the user interface, thereby confusing the
user or limiting discoverability of relevant action possibilities.''
However, the definition for \emph{Forced Action} was focused more on the
coercive nature of the interaction which may involve users' awareness
they are being manipulated: ``\emph{Forced Action} is a strategy which
requires users to perform an additional and/or tangential action or
information to access (or continue to access) specific functionality,
preventing them from continuing their interaction with a system without
performing that action.''

\subsection{Meso-Level Patterns}\label{meso-level-patterns}

\begin{quote}
\textbf{\{MESO-LEVEL DARK PATTERN\}} subverts the user's expectation
that \textbf{\{EXPECTATION\}}, instead producing or informing
\textbf{\{DIFFERENT EFFECT ON USER\}}.
\end{quote}

Across our 24 meso-level pattern definitions, we considered a range of
\emph{user expectations} such as: presence of relevant and timely
information, match between user goal and action, completeness and
truthfulness of information provided, and the ability to change one's
mind and reverse a decision. We also considered a range of
\emph{potential negative effects} on the user, such as: unexpected or
unanticipated outcomes, confusion or pressure, being prevented from
locating relevant information, or making a different choice than they
would otherwise make. Meso-level definitions as a set touched on many
different aspects of the user experience, with some pointing more
towards static moments in the user journey and others describing
temporal effects that might be realized over a longer portion of the
user journey. For instance, these two patterns represent instances where
the focus was primarily on static UI elements or a particular moment of
interaction:

\begin{itemize}
\item
  ``\emph{Manipulating Visual Choice Architecture} subverts the user's
  expectation that the options presented will support their desired
  goal, instead including an order or structure of options that makes
  another outcome more likely.''
\item
  ``\emph{Scarcity or Popularity Claims} subverts the user's expectation
  that information provided about a product's availability or
  desirability is accurate , instead pressuring the user to purchase a
  product without additional reflection or verification.''
\end{itemize}

In contrast, other patterns represented instances where the full effect
of the pattern was felt over time and might involve multiple
interactions with a system that accumulate to achieve the overall
effect:

\begin{itemize}
\item
  ``\emph{Roach Motel} subverts the user's expectation that an action
  will be as easy to reverse as it is to make, instead creating a
  situation that is easy to get into, but difficult to get out of.''
\item
  ``\emph{Hiding Information} subverts the user's expectation that all
  relevant information to make an informed choice will be available to
  them, instead hiding information or delaying the disclosure of
  information until later in the user journey that may have led to them
  making another choice.''
\end{itemize}

\subsection{Low-Level Patterns}\label{low-level-patterns}

\begin{quote}
\textbf{\{LOW-LEVEL DARK PATTERN\}} uses \textbf{\{RELATED HIGH- AND
MESO-LEVEL DARK PATTERN\}} to \textbf{\{ELEMENT OF UI ALTERED\}}. As a
result, \textbf{\{INCORRECT USER EXPECTATION\}} leads to
\textbf{\{UNDESIRED EFFECT ON USER\}}.
\end{quote}

Across our 35 low-level definitions, we considered a range of
\emph{means of execution} in the UI or user experience, such as:
provision of information that is conflicting, prohibiting certain kinds
of interactions, adding items without a user's knowledge, providing
incomplete or misleading information, distracting a user through
extraneous cues, or using social or other extrinsic pressure to steer
user's decisions. These means of execution were supported by a wide
range of \emph{incorrect user expectations and related undesired
effects}, including: preventing a user from making an informed choice
about their privacy or purchase of a product, disclosing incomplete or
misleading information that leads to choices the user would not
otherwise make, or distracting a user and thus preventing them from
discovering information that would be relevant to their decision.
Low-level patterns all exploit the user experience in direct ways, but
address different aspects of the experience:

\begin{itemize}
\item
  Focus on specific user interactions that are limited (e.g.,
  ``\emph{Price Comparison Prevention} Creates Barriers and uses
  Obstruction by excluding relevant information, limiting the ability of
  a user to copy/paste, or otherwise inhibiting a user from comparing
  prices across two or more vendors. As a result, the user cannot make
  an informed decision about where to buy a product or service.'')
\item
  Focus on a coordinated set of user interactions that produce the
  desired effect (e.g., ``\emph{Privacy Mazes} Add Steps and use
  Obstruction to require a user to navigate through many pages a result,
  the user is prevented from easily discovering relevant information or
  action possibilities, leaving them unable to make informed decisions
  regarding their privacy.'')
\item
  Focus on discrete UI elements (e.g., ``\emph{False Hierarchy}
  Manipulates the Visual Choice Architecture, using Interface
  Interference to give one or more options visual or interactive
  prominence over others, particularly where items should be in parallel
  rather than hierarchical. As a result, the user may misunderstand or
  be unable to accurately compare their options, making a selection
  based on a false or incomplete choice architecture.'')
\item
  Focus on user comprehension of the interface (e.g., ``\emph{Wrong
  Language} leverages Language Accessibility, using Interface
  Interference to provide important information in a different language
  than the official language of the country where users live. As a
  result, the user will not have access to relevant information about
  their interaction with the system and their ability to choose, leading
  to uninformed decisions.'')
\end{itemize}

\section{Extending the Ontology Based on Current and Future
Scholarship}\label{extending-the-ontology-based-on-current-and-future-scholarship}

Dark patterns researchers have addressed the impact of manipulative,
deceptive, and coercive design in a range of technological domains.
While these efforts are important in protecting online users and
identifying areas for regulatory or legal impact, the novelty and
breadth of this work potentially hinders an exhaustive mapping of dark
patterns onto our ontology. Building on our proposed ontology, we
identify pathways for many stakeholders to contribute to the growth of
ontology elements---both through the addition of new patterns and
strengthening contextual or domain-specific examples of existing
patterns. This extension can help not only to anchor instances of
patterns from future studies in existing literature, but also to enable
the scholarly community to extend or further characterize these pattern
types. The ontology's stratification allows anyone to extend the current
framework by following the structure and syntax given for each high,
meso, and low level dark pattern type.

To perform this mapping and extension exercise, we sought to identify
existing alignment between proposed dark patterns and the ontology and
also consider how a source might offer new perspectives or novel
examples of dark patterns. The method we used to extend the ontology
involves three steps:

\begin{enumerate}
\item
  We analyzed the dark pattern definition included by the author and, if
  provided, considered any cited relationships to other dark patterns
  and related terminologies.
\item
  We then aligned the author's definition with the syntax of the high,
  meso, and low levels, placing the dark pattern at the most logical
  level of abstraction.
\item
  Finally, we considered how the addition of the type informs a revision
  of the ontology. A type could reiterate an existing type in the
  ontology (leaving the core ontology unchanged), extend an existing
  type in the ontology (providing rationale for a more expansive
  definition of an existing type), or identify the presence of a wholly
  new type (adding a type to the core ontology).
\end{enumerate}

This section demonstrates how we envision for the community to extend
the ontology by drawing examples from three contemporary studies
defining dark patterns from domain and context-specific areas,
underlining the decision behind selecting these relevant work. We also
show how the ontology can be extended to map legislation and case law
relating to dark patterns.
Table~\hyperref[tab:extending-ontology]{{[}tab:extending-ontology{]}}
summarizes how three different sources were compared to our ontology
through this method, demonstrating how the ontology could be extended by
the community over time. We plan to host the ontology on a website which
will include community-vetted changes over time that follow this process
in a public, deliberative manner. Future versions of the ontology will
also be versioned and include a version history for citation accuracy.

\subsection{Dark Patterns In Non-Western Cultural
Contexts}\label{dark-patterns-in-non-western-cultural-contexts}

Hidaka et al.~\cite{hidaka2023-la} studied dark patterns in Japanese
apps and identified two dark pattern types---``untranslation'' and
``alphabet soup''---which are sub-types of a novel ``linguistic
dead-end'' dark pattern. We closely evaluated the authors' definition of
\emph{Linguistic Dead-End}, where use of a foreign language hinder users
from understanding the consequences of their interactions. When
comparing these three patterns to our ontology, the high-level pattern
\emph{Linguistic Dead-End} appears to fit within the existing meso-level
dark pattern \emph{Language Inaccessibility}, while extending its
coverage. The remaining two low-level patterns, \emph{Untranslation} and
\emph{Alphabet Soup}, can then be nested as two low-level types
underneath the same meso-level dark pattern, with \emph{Untranslation}
mapping to and extending the existing \emph{Wrong Language} dark pattern
and \emph{Alphabet Soup} forming a new low-level pattern. In this case,
the three dark patterns extend and further support a distinct area of
the ontology, demonstrating how novel contexts help to usefully
supplement existing dark patterns and identify new low-level means of
execution.

\subsection{Contextual Dark Patterns in Different Screen
Modalities}\label{contextual-dark-patterns-in-different-screen-modalities}

Gunawan et al~\cite{Gunawan2021-pr} investigated the presence of dark
patterns across different screen modalities, describing eight novel dark
pattern types which limit the choices of users depending on the device
used. In the provided definitions for each proposed dark pattern, the
authors included links to previously defined dark patterns---linking
these patterns to elements of the ontology, thus providing an easy
mapping path. The \emph{Extraneous Badges} dark pattern, for example, is
indicated as related to \emph{Aesthetic Manipulation}~\cite{Gray2018-or}
as a form of \emph{Interface Interference}, and would result in this
dark pattern being included as a new low-level type in the ontology.
Similarly, using the authors' definitions and identification of mapping
in the paper text, \emph{Account Deletion Roadblocks} could extend
\emph{Roach Motel} through two specific new low-level types focusing
variously on insufficient communication and time delay: \emph{Unclear
Deactivation/Deletion Options} and \emph{Time-Delayed Account Deletion}.
These examples illustrate how contextual and situational links to
previously defined dark patterns support the ontology, describing
specific situations that strengthen established dark patterns and
identify new low-level means of execution.

\subsection{Domain-Specific Dark Patterns in Social Media
Applications}\label{domain-specific-dark-patterns-in-social-media-applications}

Mildner et al.~\cite{Mildner2023-ab} investigated dark patterns on
social media platforms, proposing five dark patterns across two
strategies. As with Hidaka et al., the granularity of their definitions
imply a mapping on multiple levels of the ontology. We began by drawing
from the authors' definitions of \emph{Engaging Strategies} and
\emph{Governing Strategies}. The authors describe the aim of
\emph{Engaging Strategies} as entertaining users for as long as
possible, related to \emph{Attention
Capture}~\cite{monge_roffarello2023-ac}, which is already included in
the ontology as a meso-level pattern under \emph{Forced Action}.
However, some elements of the original definition (e.g., occupying and
entertaining) fit more closely within concepts of \emph{Social
Engineering}. Similarly, \emph{Governing Strategies} can be partially
linked to multiple patterns in the ontology. For example, as the authors
originally suggest, the strategy can be enabled through \emph{Interface
Interference}. However, \emph{Governing Strategies} also offers a
high-level focus to inspect \emph{Obstruction} with \emph{Labyrinthine
Navigation}, presenting an interesting adaption of \emph{Privacy Maze}
already present in the ontology. These examples indicate how the authors
make their dark pattern types distinct from prior ones, functioning as a
lens that might invite reinspection of dark patterns in the ontology and
perhaps indicate opportunities for further development of low-level
patterns.

\subsection{Dark Patterns in Legislation and Case
Law}\label{dark-patterns-in-legislation-and-case-law}

An alignment between legislation, the ontology, and case law shows that
it could also be a robust and reliable artifact for regulators and
policy makers to use in their compliance monitoring and enforcement
actions.

\textbf{Mapping the ontology to case law} Dark patterns have been
detected in regulatory cases by enforcers, such as Data Protection
Authorities (DPAs) and Consumer Protection Authorities, for more than a
decade~\cite{FTC2022,EUCOM2022}. However few cases explicitly designate
dark patterns as such.\footnote{Case law and legal frameworks have
  recently been added to the \url{https://deceptive.design} site, which
  include mappings to specific dark
  patterns.~\cite{deceptivedesign-legalcases}} Decisions analyse several
practices that are related to dark patterns, but without qualifying each
practice into a concrete granular type of dark pattern. Current case law
descriptions of the use of dark patterns often report infringements only
at a general level, but without qualifying each practice as a concrete
type of dark pattern~\cite{Santos_Rossi_2023}. In doing so, case law
could miss lower-level granularity that may translate across domains. A
recent example shows that a EU regulator, the Italian DPA, used the
concept of dark patterns related to certain consent practices for the
first time in an official EU legal
decision~\cite{ItalianDPAvsEdiscom2023}. By mapping case law to the
ontology, regulators can gain additional knowledge identifying where
dark patterns practices at multiple levels and in multiple combinations
are at play, and were deemed to be illegal per
jurisdiction~\cite{Leiser-2022-regpluralismGDPR/UCPD}, enhancing legal
certainty about dark patterns practices. For example, the EU Court of
Justice has ruled that the practice called ``pre-selection'' violates
the GDPR~\cite{CJEU-Planet49-19}, which maps to the meso-level dark
pattern \emph{``Bad Defaults''} in our ontology. Further, the ontology
has the potential to support enforcement decisions since it can test and
confirm the traceability of concrete dark patterns-related practices.
For instance, the Italian Data Protection Authority has already added
the keyword ``dark pattern'' to the available tags of their online
database\footnote{\url{https://www.garanteprivacy.it/temi/internet-e-nuove-tecnologie/dark-pattern}}---a
useful effort that should be extended to official and unofficial
searchable databases of enforcers' decisions. Connecting case law to
multiple levels of dark patterns in our proposed ontology has the
potential to inform enforcers of different jurisdictions in the EU/US
and reduce the risks of gaps or overlaps.

\textbf{Mapping the ontology to legislation} The proposed ontology can
also help regulators across different jurisdictions to understand
relationships between different definitions of dark patterns, including
high-, meso- and low level dark patterns, including when such
definitions map to existing and upcoming legislation. The recent EU
Digital Service Act (DSA)\cite[Art.25(3)(b), recital 67]{DSA2022}
explicitly prohibits user manipulation and specifies that further
guidelines will be given on a specific practice, where ``repeatedly
requesting that the recipient of the service make a choice where that
choice has already been made, especially by presenting pop-ups that
interfere with the user experience''; this example maps well to the
proposed {\emph{Nagging}} dark pattern in our ontology. Because new
legislation, such as the DSA\cite{DSA2022}, Data Market Act
(DMA)\cite{DMA}, Data Act \cite{Data-Act-proposal}, and California
CPRA~\cite{CPRA} contain dark patterns specific prohibitions, we believe
the proposed ontology has the capability to ensure a precise mapping
between the concepts of dark patterns in research literature and the
legally-binding provisions. When the concepts of the ontology are mapped
to a legal concept, then it is easier for regulators to link a specific
dark pattern to a concrete binding legislative provision. Consequently,
the ontology will help to conclude the normative value of such
practice---whether a specific dark pattern is illegal or legal---and
what relevant obligations and rights are derived from the law and must
be enforced. If regulators and policy-makers across jurisdictions rely
on the same definitions of dark patterns, this can assure an easier
re-use of case law for future legal cases.

\section{Using the Ontology to Support Transdisciplinary
Engagement}\label{using-the-ontology-to-support-transdisciplinary-engagement}

In this ontology, we seek to synthesize and harmonize existing academic
and regulatory taxonomies while adding useful and consistent structure
to allow for other stakeholders to build upon and derive benefit from a
shared description of dark patterns knowledge. This paper lays the
foundation for shared action, which includes many different stakeholders
with differing aims. In this section, we outline key opportunities for
future transdisciplinary engagement, identifying opportunities for
scholars to continue building knowledge about dark patterns and their
harms, for regulators and other enforcement agencies to better detect
and thus sanction dark patterns, and for legal scholars and legislators
to address current and future consequences of dark patterns that can
inform further action.

\subsection{Challenges in Evolving the
Ontology}\label{challenges-in-evolving-the-ontology}

Not all of our mappings were clear-cut and some may be productively
extended or disputed in future versions of this ontology. Through
dialogue, we sought to locate existing patterns within our ontology
based on our best understanding of the pattern as described by its name
and definition in the source taxonomy. One challenge we faced was that
some combinations of patterns have evolved over time. For instance,
Mathur et al.'s~\cite{Mathur2019-hx} high-level pattern ``social proof''
originated with two sub-patterns, ``activity messages'' and
``testimonials.'' Later, the FTC created new low-level patterns,
introducing ``endorsements'' (we bundled it with testimonials as one
low-level pattern) and more specific types of endorsement or
testimonials (e.g., ``deceptive celebrity endorsements,'' ``false
activity messages''). Future work could identify the most useful level
of abstraction for these patterns. Additionally, the use of novel names
for patterns (particularly by the EDPB and CMA) or the use of patterns
in specific contexts (e.g., e-commerce, social media) caused us to
consider both the presence of granular low-level patterns and the
relation of these low-level patterns to inferred meso-level patterns. In
particular, the use of novel names for patterns types and definitions
was a challenge from an analytic perspective, resulting in: i) instances
where a wholly new pattern was introduced (e.g., CMA's ``information
overload'' which we leveraged to create a new meso-level pattern of
``choice overload''); ii) instances where a new high-level strategy was
highly similar to an existing high-level strategy (e.g., EDPB's
``skipping'' which we subsumed within ``sneaking''); and iii) instances
where existing patterns included both a generalizable pattern and
domain-specific information which may need to be captured in specific
low-level patterns in future work (e.g., EDPB's ``left in the dark'' is
a form of ``hidden information'' but implies specific low-level patterns
that are specific to data protection). These observed challenges point
towards the value of a shared ontology that includes a consistent
vocabulary, but also points to opportunities to generate more specific
knowledge that is linked to particular contexts and technologies. For
instance, low-level patterns could be tagged based on how well they
relate to specific contexts (e.g., e-commerce, social media),
technologies (e.g., CUIs, VR/AR, robots), or application domains (e.g.,
health, travel) as indicated by a recent systematic review of dark
patterns literature~\cite{Gray2023-systematic}.

\subsection{Activating Transdisciplinary
Pathways}\label{activating-transdisciplinary-pathways}

As we have outlined, work relating to dark patterns has connected many
different disciplinary communities toward shared goals, including social
scientists studying the presence and harms of dark patterns, legal
scholars linking instances of dark patterns to relevant consumer
protection or data protection legal frameworks, legislators targeting
specific legal provisions about dark patterns to support new obligations
and/or future sanctions, and regulators detecting legal violations
related to dark patterns to support enforcement sanctions. We consider
multiple opportunities for collaboration within and across these
stakeholder groups:

\begin{itemize}
\item
  \textbf{Social Scientists} Scientists studying dark patterns can use
  the ontology to better map the impact triggered by certain dark
  patterns in concrete contexts in ways that support shared knowledge
  building and reduce duplication. This approach has been applied for
  specific low-level patterns by various empirical studies that
  evaluated the impact of dark pattern design on the outcome of users'
  consent decisions~\cite{Biel-LINC-2023}, but could be scaled up
  substantially using the ontology as a means of producing and sharing
  these mappings.
\item
  \textbf{Social Scientists + Computer Scientists} The detection of dark
  patterns could also be more robustly supported by our ontology, with
  our assertion that low-level patterns show the most promise in being
  detectable. Existing detection efforts
  (e.g.,~\cite{Stavrakakis2021-hz,Soe2022-lt,Mathur2019-hx,Nouwens2020-ij,hofslot-2022-AutomaticClassifViolCookieBanners,chen2023-ut,Bouhoula-2023,Koch-2023,Yada2022-he})
  have shown that higher-level patterns are difficult or impossible to
  detect at scale due to their abstract nature that requires
  interpretation, while low-level UI elements with discrete and known
  qualities (e.g., cookie consent banners, elements of the checkout
  process) are more detectable using software tools for automated
  detection. Our ontology of low-level patterns and gaps creates a
  foundation for future detection efforts, allowing computer science
  scholars to focus on pattern types which are most likely to be
  detectable and measurable.
\item
  \textbf{Social Scientists + Regulators} Bielova et
  al.~\cite{Bielova2024-zr} have recently compared the results of such
  empirical studies and designs recommended by EU regulators and found
  multiple gaps and contradictions relating to instances of dark
  patterns, showing that empirical studies bring important insights not
  only in the research community but also for the regulators and
  policy-makers. This effort demonstrates an opportunity for regulators
  and social scientists to work more closely---commissioning studies
  where user experience of dark patterns is unknown or unclear
  (particularly with relation to causal mechanisms) while deprioritizing
  studies that address design choices that are already illegal under
  statute.
\item
  \textbf{Social Scientists + Legal Scholars} The ontology can be
  extended to consider potential harms in relation to specific dark
  patterns types~\cite{Gunawan2022-harms}. For example, the meso-level
  dark pattern \emph{Nagging} can arguably trigger ``attentional
  theft,'' thus harming consumer welfare, and can lead to indirect harms
  such as increased vulnerability to privacy violations, and finally, to
  anti-competitive harms~\cite{Hung-nagging}. A mapping of harms to
  specific types of dark patterns in the ontology may support
  connections to avenues for legal remedies, as well as aid in
  identifying areas where additional research is needed.
\item
  \textbf{Legal Scholars + Regulators} The ontology may also be extended
  to refer to concrete enforcement cases already consolidated in a
  database of dark patterns case law, such as those on Brignull's
  updated site~\cite{deceptivedesign-legalcases}. This will allow for
  case law to inform future legal sanctions, identify which elements of
  the ontology connect to existing legal frameworks, and lay the
  groundwork for future legislative action to allow for sanctioning of
  novel patterns that are not well addressed through existing laws.
\end{itemize}

\section{Conclusion}\label{conclusion}

To support the development of a shared language of dark patterns, in
this paper we present our analysis of ten existing regulatory and
academic taxonomies of dark patterns and propose a three-level ontology
with standardized definitions for 65 synthesized dark pattern types
across low-, meso-, and high-level patterns. Building on our analysis,
future scholars, regulators, and legal professionals can benefit from
our hierarchical organization of dark patterns types to indicate links
to existing and similar concepts. This description encourages the
establishment of provenance in future work, allowing scholars and
regulators to identify pattern types and their origins and provide an
audit trail to connect specific contextually-bound instances with
broader categorizations. This ontology creates a foundation for a shared
and reusable knowledge source, allowing many stakeholders to work
together in building a shared, explicit and precise conceptualization of
what is already known in the literature and which can be further refined
and extended. Finally, we illustrate how this ontology can support
translational research and regulatory action, by extending the ontology
from three contemporary studies defining dark patterns from domain and
context-specific areas, as well as ontology extension to map legislation
and case law.

This work is funded in part by the National Science Foundation under
Grant No. 1909714 and the ANR 22-PECY-0002 IPOP (Interdisciplinary
Project on Privacy) project of the Cybersecurity PEPR.


==> olddiscussion.tex <==
\subsection{Evolving of the Ontology %Opportunities for Further Development
}
Not all of our mappings were clear-cut and some may be productively extended or disputed in future versions of this ontology. Through dialogue, we sought to locate existing patterns within our ontology based on our best understanding of the pattern as described by its name and definition in the source taxonomy. We describe some of our challenges in mapping and present these as opportunities to refine the ontology in future work: %Some ambiguous cases are discussed herewith.


\textbf{Combinations of patterns evolve over time.} Some combinations of patterns have evolved over time. For instance, Mathur et al.'s~\cite{Mathur2019-hx} high-level pattern ``social proof'' originated with two sub-patterns, ``activity messages'' and ``testimonials.'' %However, 
%
The FTC created new low-level patterns, introducing ``endorsements'' (we bundled it with testimonials as one low-level pattern) and more specific types of endorsement or testimonials (e.g., ``deceptive celebrity endorsements,'' ``false activity messages''). 
Future work could identify the most useful level of abstraction for these patterns.
%
\CS{Thomas your input on time bounded DP is very useful here --pls include}


\textbf{Novel and context-specific names for dark patterns have been introduced.} The use of novel names for patterns (particularly by the EDPB and CMA) or the use of patterns in specific contexts (e.g., e-commerce, social media) caused us to consider both the presence of granular low-level patterns and the relation of these low-level patterns to inferred meso-level patterns. 
%
%\CS{what about introducing a case study paragraph with new categories and intersection with other taxonomies? below}
In particular, the use of novel names for patterns types and definitions was a challenge from an analytic perspective, resulting in: 
i) instances where a wholly new pattern was introduced (e.g., CMA's ``information overload'' which we leveraged to create a new meso-level pattern of ``choice overload''); %(e.g., EDPB's ``dead end'', a low-level which we subsumed within ``roach motel''); 
ii) instances where a new high-level strategy was highly similar to an existing high-level strategy (e.g., EDPB's ``skipping'' which we subsumed within ``sneaking''); and iii) instances where existing patterns included both a generalizable pattern and domain-specific information which may need to be captured in specific low-level patterns in future work (e.g., %instances where multiple patterns had similarities and infer the space for a set of low-level patterns that are not sufficiently defined in any existing definitions 
%(e.g., the EDPB's ``deceptive snugness'' as a form of ``preselection'', which we subsumed under the ``bad defaults'' meso-level pattern (however, the former is more domain-related to data-invasive behaviors); 
EDPB's ``left in the dark'' is a form of ``hidden information'' but implies specific low-level patterns that are specific to data protection).%, but which could result in a finer distinction at the low-level of instances where information is hidden to delay divulging of important information versus information that is hidden to confuse the user). 



\textbf{Engaging in more robust citation practices to trace the evolution of pattern types and their presence over time.} 
%\CS{looks much more tuned to 8.1 regarding traceability over time; let's move? }
This ontology---and its extension over time---can be supported through robust citation patterns across regulatory and academic literature, including indications where definitions of specific patterns have been altered, extended, or synthesized. While definitions of some low and high-level patterns have remained relatively consistent over time (in particular, Brignull's original patterns), the rapid growth of new pattern types and the introduction of hierarchy injects added complexity that can inform more disciplined and transparent knowledge generation practices. % with clear links to past scholarship.





%\subsection{Problematizing the Ontology} Situating the Onotlogy in the Dark Pattern  Discourse
% Why We need an Ontology? -> The solutions offered by the ontology.
\subsection{Situating the ontology  through different dimensions of dark patterns.}
%e\CS{can we have another title here?}
%These analytic challenges strengthen some of the key definitional components of dark patterns as they have previously been described in the literature~\cite{Mathur2021-rc} but inform areas where definitions could be further problematized. 

Further alignment of dark patterns definitions can be achieved through multiple dimension of dark patterns %types of practices 
that could further help establish dialogue between actors from different disciplinary and professional roles.
In fact, many pattern definitions mixed \textit{characteristics} of dark patterns (e.g., information hiding, manipulation of the choice architecture), 
\textit{impact on user behavior} (e.g., confusion, obstruction), \textit{manifestation in the user interface} (e.g., visibility of elements, interpretability by users), and 
\textit{context-specific issues} (e.g., impacts on data protection, presentation in social media interfaces). 
%
Future definitions of patterns at all levels could benefit from separating out these elements at appropriate levels of abstraction to increase the potential for utility across many contexts and domains---particularly at the high- and meso-levels of pattern description.
%%%%
%%%%%
%For instance, many regulatory definitions tended to mix characteristics of dark patterns (e.g., information hiding, manipulation of the choice architecture), impact on user behavior (e.g., confusion, obstruction), manifestation in the user interface (e.g., visibility of elements, interpretability by users), and context-specific issues (e.g., impacts on data protection, presentation in social media interfaces). Future definitions of patterns at all levels could benefit from separating out these elements at appropriate levels of abstraction to increase the potential for utility across many contexts and domains---particularly at the high- and meso-levels of pattern description.


\subsection{Identifying multiple levels of granularity.} %First, 
This ontology can be used to identify abstractions of dark patterns across many domains, contexts, or application types (i.e., high- and meso-level patterns) while creating more robust characterizations of low-level patterns that may be highly domain or context specific. 
%
%Our indication of gaps in our draft ontology shows that many additional low-level patterns need to be identified to allow for more precise detection techniques and guidance for designers. For instance, ``nagging'' only exists as a high-level pattern and it is unclear which kinds of nagging should be considered problematic, under which conditions, and in relation to specific harms. 
%By indicating gaps in our draft ontology, we show that many additional low-level patterns need to be identified, which would aid computer scientists and engineers in building precise detection tools and provide guidance for designers. 
%
%For instance,
%We posit that {\em Nagging} only exists as a meso-level dark pattern, however it is unclear which kinds of nagging should be considered problematic, and under which conditions.
%
%Also, the ontology can be further made more granular to include potential harms in relation to specific dark patterns types~\cite{Gunawan2022-harms}. %and in relation to specific harms. 
%
Other meso-level patterns that lack any defined low-level patterns (e.g., ``trick questions,'' ``choice overload,'' ``hidden information'') %, ``feedforward ambiguity'')% ``forced continuity,'' ``forced registration,'' and ``attention capture'' 
raise the question of which specific cases---as inscribed through low-level patterns---need to be articulated as particularly problematic or indicative. This work will require a shared language among regulators and scholars to inform disciplined inquiry of specific domains and use contexts.

%\CS{Can we say that the ontology-- each type of DP type-- could be populated/characterized according to more related data types, e.g. the harms it (or a combo) might cause; remedies associated per type(s); known vulnerability drivers exploited per type, most impacted people? most effective dark patterns; and the users perceptions (even mapping to user studies); or even mapping to other domain-DP taxonomies}






\subsection{Using levels of pattern granularity to inform the detection of dark patterns through automated or manual approaches.} 
The detection of dark patterns could also be more robustly supported by our ontology, with our assertion that low-level patterns show the most promise in being detectable. Existing detection efforts (e.g.,~\cite{Stavrakakis2021-hz,Soe2022-lt,Mathur2019-hx,Nouwens2020-ij,hofslot-2022-AutomaticClassifViolCookieBanners,chen2023-ut,Bouhoula-2023,Koch-2023,Yada2022-he}) have shown that higher-level patterns are difficult or impossible to detect at scale due to their abstract nature that requires interpretation, while low-level UI elements with discrete and known qualities (e.g., cookie consent banners, elements of the checkout process) are more %readily accessible through the Document Object Model (DOM) and are thus able to be modeled. 
accessible with software tools for automated detection.
Our ontology of low-level patterns and gaps creates a foundation for future detection efforts, allowing % web measurement scholars 
computer science scholars 
to focus on pattern types which are most likely to be detectable.


%\textcolor{red}{Relationship effects---e.g., amplification, etc.}

%\CS{X manifestations so far, and this number continues to grow according to new domains/sectors -- how can this high/meso/low level O be sustainable/manageable?}

==> ontology-workingdefs.tex <==
\begin{itemize}
    \item \textbf{Nagging} is a strategy which \textbf{repeatedly interrupts the user during normal interaction,} that 
    %\textbf{distracting the user from a desired task by foregrounding tasks not directly related to the one the user is focusing on.}
    \textbf{distracts the user from a desired task the user is focusing on to induce an action or make a decision the user does not want to make.}
    \item \textbf{Sneaking} is a strategy which \textbf{hides, disguises, or delays the disclosure of important information} that, if made available to users, 
    %\textbf{they would likely object to}.
    \textbf{would cause a user to unintentionally take an action they would likely object to.}
        \begin{itemize}
            \item \textbf{Bait and Switch} subverts the user's expectation that {their choice will result in a desired action}, instead leading to 
            {an unexpected, undesirable outcome}.
            \item \textbf{Hiding Information} subverts the user's expectation that {all relevant information to make an informed choice will be available to them}, instead {hiding information or delaying the disclosure of information until later in the user journey that may have led to them making another choice}.
            \item \textbf{(De)contextualizing Cues} subverts the user's expectation that {provided information will guide the user to making an informed choice}, instead {confusing the user and/or preventing them from locating relevant information due to the context where information is presented}. 
            \begin{itemize}
                \item \textbf{Information without context} uses \textbf{(De)contextualizing Cues} and \textbf{Sneaking}
                to \textbf{relevant information or control}. 
                As a result, \textbf{} 
                \textbf{users are unlikely  to  find  the  information  or  control they are interested in}.
            \end{itemize}
        \end{itemize}
        
    \item \textbf{Obstruction} is a strategy which \textbf{impedes a user's task flow, making an interaction more difficult than it inherently needs to be,} \textbf{dissuading a user from taking an action}.

        \begin{itemize}
            \item \textbf{Roach Motel} subverts the user's expectation that an action will be as easy to reverse as it is to make, instead creating a situation that is easy to get into, but difficult to get out of.
            
            \item \textbf{Creating Barriers} subverts the user's expectation that relevant user tasks will supported by the interface, instead preventing, abstracting, or otherwise complicating a user task to disincentive user action.
            
            \item \textbf{Adding Steps} subverts the user's expectation that a task will take as few steps as technologically needed, instead creating additional points of unnecessary but required user interaction to perform a task.
        \end{itemize}
        
    \item \textbf{Interface Interference} is a strategy which \textbf{privileges specific actions over others through manipulation of the user interface,} thereby \textbf{confusing the user or limiting discoverability of relevant action possibilities.}

        \begin{itemize}
            \item \textbf{Manipulating Visual Choice Architecture} subverts the user's expectation that the options presented will support their desired goal, instead including an order or structure of options that makes another outcome more likely.
            
            \item \textbf{Bad Defaults} subverts the user's expectation that default settings will be in their best interest, instead requiring users to take active steps to change settings that may cause harm or unintentional disclosure of information.
            
            \item \textbf{Emotional or Sensory Manipulation} subverts the user's expectation that the design of the site will allow them to achieve their goal without manipulation, instead altering the language, style, color, or other design elements to evoke an emotion or manipulate the senses in order to persuade the user into a particular action.
            
            \item \textbf{Trick Questions} subvert the user's expectation that prompts will be written in a straightforward and intelligible manner, instead using confusing wording, double negatives, or otherwise leading language or interface cues to manipulate a user's choice.
            
            \item \textbf{Choice Overload} subverts the user's expectation that the choices they make should be understandable and comparable, instead providing too many options to compare or encouraging users to overlook relevant information due to the volume of choices provided.
            
            \item \textbf{Hidden Information} subverts the user's expectation that relevant information will be made accessible and visible, instead disguising relevant information or framing it as irrelevant. 
            
            \item \textbf{Language Inaccessibility} subverts the user's expectation that guidance will be provided in a way that is understandable and intelligible, instead using unnecessarily complex language or a language not spoken by the user to decrease the likelihood the user will make an informed choice.
   
            \item \textbf{Feedforward Ambiguity} subverts the user's expectation that their choice will be likely to result in an action they can predict, instead providing a discrepancy between information and actions available to  users that results in an outcome that is different from what the user expects.
        \end{itemize}

    \item \textbf{Forced Action} is a strategy which \textbf{requires users to perform an additional and/or tangential action or information to access (or continue to access) specific functionality,} \textbf{preventing them from continuing their interaction with a system without performing that action}.

    \begin{itemize}
        \item \textbf{Forced Continuity} subverts the user's expectation that a subscription created in the past will not auto-renew or otherwise continue in the future, instead causing undesired charges, difficulty to cancel, or lack of awareness that a subscription is still active.
        
        \item \textbf{Forced Registration} subverts the user's expectation that they can complete an action without registering or creating an account, instead tricking them into thinking that registration is required, often resulting in the sharing of unneeded personal data.

        \item \textbf{Forced Communication or Disclosure} subverts the user's expectation that a system will only request information needed to complete their desired goals, instead tricking them into sharing more information about themselves or using their information for purposes that they do not desire.

        Privacy Zuckering tricked into publicly sharing information about themselves 
        Address Book Leeching collects data for purposes not initially declared
        Social Pyramid recruits others to use a service (i.e., social recruiting) 
        Friend Spam requests personal information used for spam or other unintended purposes
        
        \item \textbf{Gamification} subverts the user's expectation that relevant functionality is provided based on their goals, instead tricking them into ``earning'' (perhaps undesired) aspects of the service repeatedly in order to earn access to desired features.

        Pay-to-Play
        Grinding
        
        \item \textbf{Attention Capture} subverts the user's expectation that they have rational control over the time they spend using a system, instead tricking them into spending more time or other resources to continue use for longer than they otherwise would.

        Auto-Play 
        
        Automatically playing another video once one video 
ends in a manner that is unexpected or harmful 
Example: after the first video, a less kid-friendly  video – or a sponsored ad camouflaged to look  like a recommended video – automatically plays

        
    \end{itemize}

    \textbf{\{MESO-LEVEL DARK PATTERN\}} subverts the user's expectation that \textbf{\{EXPECTATION\}}, instead causing \textbf{\{DIFFERENT EFFECT ON USER\}}.

    \item \textbf{Social Engineering} is a strategy which \textbf{presents options or information that causes a user to be more likely to perform a specific action based on their individual and/or social cognitive biases,%psychological profile,
    } \textbf{thereby leveraging a user's desire to follow expected or imposed social norms.} %``fit in'' or do the ``expected thing''}.

        \begin{itemize}
            \item \textbf{Scarcity or Popularity Claims} subverts the user's expectation that information provided about a product's availability or desirability is accurate %purchasable item is not limited in stock
            , instead pressuring the user to purchase a product without additional reflection or verification. % item before reflecting on their decision as they observe that only a limited amount of a purchasable item is available or under high demand.
            % The choice architect informs consumers  about limited stock, limited time to buy, or  high popularity of an item.
            
            \item \textbf{Social Proof} subverts the user's expectation that the indicated behavior of others in a specific situation is correct or desirable, instead accelerating user decision-making and encouraging the user to trust flawed implications through provided information. % while exploiting the underlying cognitive bias of the same name.
            %According to the social proof principle, individuals determine the correct action and behavior for themselves in a given situation by examining the action and behavior of others [37,69]. The ‘Social Proof’ dark pattern uses this influence to accelerate user decision-making and purchases, exploiting the bandwagon effect cognitive bias to its advantage.
            
            \item \textbf{Urgency} subverts the user's expectation that information provided about discounts or a limited-time deal for a product is accurate, instead accelerating the user's decision-making process by demanding immediate or timely action.
            % 'Urgency' refers to the category of dark patterns that impose a deadline on a sale or deal, thereby accelerating user decision-making and purchases
            
            \item \textbf{Shaming} subverts the user's expectation that their decision is being guided by objective information and made in an informed way, %to cancel a subscription or leave a service is without consequences, 
            instead using emotionally manipulative tactics to % them to overthink their decision by applying emotional pressure and manipulation to 
            pressure the user to make certain choices over others in order for them to feel they have done the right thing.
            
            \item \textbf{Personalization} subverts the user's expectation that products or service features are offered to all users in similar ways, %objectively without misusing personal data, 
            instead using personal data to shape elements of the user experience that %create personalized offers to 
            manipulate the user's goals while hiding other %, perhaps relevant, 
            alternatives.
            %The choice architect uses data to personalise  offers.
        \end{itemize}

\end{itemize}

==> ontologytable.tex <==
\begin{table*}
\centering
\begin{tabularx}{\textwidth}{X>{\raggedright\arraybackslash} X >{\raggedright\arraybackslash} X >{\raggedright\arraybackslash}}
\toprule
High-Level Pattern (Strategy)                                                                                                                                                                                                                                                      & Meso-Level Pattern (Angle of Attack)                                                                                                                                                                      & Low-Level Pattern (Means of Execution)                                                                                                                                                                     \\
\midrule

\begin{tabular}[c]{@{}l@{}}Nagging (D:~\cite{Gray2018-or,Luguri2021-bg,EUCOM2022,FTC2022,Oecd2022}; I:~\cite[``continuous prompting'']{EDPB2022}\cite[``prompts and reminders'']{CMA2022}\end{tabular}                                                                                                                        & –                                                                                                                                                                                                         & –                                                                                                                                                                                                          \\

\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}Obstruction \\(direct: Gray, Luguri, Mathur, EUCOM, FTC, OECD; inferred: EDPB (hindering),  CMA (sludge))\end{tabular}}                                                                                                                       & \multirow{2}{*}{Roach Motel (direct: Brignull, Gray, Luguri, EUCOM); inferred: OECD (hard to cancel…), FTC (roadblocks to cancellation), Mathur (hard to cancel),  FTC  and Bösch and OECD (immortal accounts)} & Immortal Accounts (direct: FTC,  Bösch)                                                                                                                                                                     \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Dead End (direct: EDPB; inferred: most others)                                                                                                                                                             \\
                                                                                                                                                                                                                                                                                   & \multirow{2}{*}{Creating Barriers}                                                                                                                                                                        & Price Comparison Prevention (direct: FTC,  EUCOM, Brignull, Gray, Luguri, OECD)                                                                                                                                 \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Intermediate Currency (direct: Gray, FTC, Luguri, EUCOM, OECD; inferred: CMA (virtual currencies in gaming)                                                                                                    \\
                                                                                                                                                                                                                                                                                   & Adding Steps (inferred: EDPB (longer than necessary))                                                                                                                                                     & Privacy Maze (direct: EDPB)                                                                                                                                                                                \\
                                                                                                                                                                                                                                                                              
                                                                                                                                                                                                                                                                             \midrule

\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Sneaking \\(direct: Gray, Luguri, Mathur, EUCOM, OECD; inferred: FTC (sneaking or information hiding),  EDPB (skipping),  CMA (dark nudge))\end{tabular}}                                                                                     & Bait and Switch (direct: EUCOM, FTC, Luguri, Brignull, Gray; inferred: OECD (bait and switch,  including bait pricing)                                                                                         & Disguised Ad (direct: FTC, Brignull, Gray, OECD, EUCOM, Luguri)                                                                                                                                                 \\
                                                                                                                                                                                                                                                                                   & \multirow{2}{*}{Hiding Information}                                                                                                                                                                       & Sneak into Basket (direct: Brignull,  Mathur, FTC, EUCOM, Gray, Luguri, OECD)                                                                                                                                    \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Drip Pricing,  Hidden Costs,  or Partitioned Pricing (direct: FTC and CMA (drip pricing); EUCOM, Brignull, FTC, Gray, Mathur, Luguri (hidden costs); OECD (hidden costs/drip pricing); CMA (partitioned pricing)  \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Reference Pricing (direct: CMA, OECD)                                                                                                                                                                       \\
                                                                                                                                                                                                                                                                                   & \multirow{2}{*}{(De)contextualizing Cues}                                                                                                                                                                 & Conflicting Information (direct: EDPB)                                                                                                                                                                     \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Information without Context (inferred: EDPB (decontextualizing)                                                                                                                                            \\
\midrule
\multirow{13}{*}{\begin{tabular}[c]{@{}l@{}}Interface Interference \\(direct: FTC, Gray, Luguri, EUCOM, OECD; indirect: EDPB (stirring + overleading + fickle),  FTC (asymmetric choice + misdirection),  Mathur (visual interference),  Brignull and Mathur (misdirection)\end{tabular}} & \multirow{4}{*}{Manipulating Visual Choice Architecture (inferred: CMA (framing + ranking)}                                                                                                               & False Hierarchy (direct: Bösch, Gray,  FTC,  Luguri, OECD; inferred: EDPB (lacking hierarchy))                                                                                                                 \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Visual Prominence (inferred: EDPB (look over there))                                                                                                                                                       \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Bundling (direct: CMA)                                                                                                                                                                                     \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Pressured Selling (direct: FTC, Luguri)                                                                                                                                                                     \\
                                                                                                                                                                                                                                                                                   & Bad Defaults (direct: FTC, OECD, Luguri, Gray; inferred: EUCOM (preselection (default)),  EDPB (deceptive snugness),  CMA (defaults))                                                                          & –                                                                                                                                                                                                          \\
                                                                                                                                                                                                                                                                                   & \multirow{2}{*}{Emotional or Sensory Manipulation (inferred: Gray,  Luguri, EUCOM, OECD (toying with emotion); CMA (sensory manipulation))}                                                                  & Cuteness (direct: Luguri)                                                                                                                                                                                  \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Positive or Negative Framing (inferred: Gray (aesthetic manipulation),  EDPB (emotional steering))                                                                                                          \\
                                                                                                                                                                                                                                                                                   & Trick Questions (direct: Brignull, Gray, Mathur, Luguri, EUCOM, OECD, FTC)                                                                                                                                      & –                                                                                                                                                                                                          \\
                                                                                                                                                                                                                                                                                   & Choice Overload (inferred: EDPB (too many options),  CMA (choice overload and decoys + information overload)                                                                                               & –                                                                                                                                                                                                          \\
                                                                                                                                                                                                                                                                                   & Hidden Information (direct: Luguri, EUCOM, FTC, Gray, OECD; inferred: EDPB (left in the dark + hidden in plain sight))                                                                                        & –                                                                                                                                                                                                          \\
                                                                                                                                                                                                                                                                                   & \multirow{2}{*}{Language Inaccessibility}                                                                                                                                                                 & Wrong Language (inferred: EDPB (language discontinuity))                                                                                                                                                   \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Complex Language (direct: CMA)                                                                                                                                                                             \\
                                                                                                                                                                                                                                                                                   & Feedforward Ambiguity (inferred: EDPB (ambiguous wording or information + misleading information))                                                                                                        & –                                                                                                                                                                                                          \\
\midrule
\multirow{9}{*}{\begin{tabular}[c]{@{}l@{}}Forced Action \\(direct: Gray, Luguri, EUCOM, Mathur, OECD; inferred: CMA (forced outcomes),  FTC (coerced action))\end{tabular}}                                                                                                            & Forced Continuity (direct: Brignull, Gray, EUCOM, Luguri,  FTC, OECD; inferred: Mathur (hidden subscription))                                                                                                  & –                                                                                                                                                                                                          \\
                                                                                                                                                                                                                                                                                   & Forced Registration (direct: Luguri, EUCOM, OECD, FTC; inferred: Mathur (forced enrollment),  CMA (commitment), FTC (unauthorized transactions))                                                               & –                                                                                                                                                                                                          \\
                                                                                                                                                                                                                                                                                   & \multirow{4}{*}{Forced Communication or Disclosure}                                                                                                                                                       & Privacy Zuckering (direct: Gray, Brignull, Luguri, OECD; inferred: FTC (subverting privacy preferences))                                                                                                      \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Friend Spam (direct: FTC, Brignull, Luguri, OEC)                                                                                                                                                              \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Address Book Leeching (direct: FTC, Luguri, OECD)                                                                                                                                                            \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Social Pyramid (direct: Gray, FTC, Luguri, OECD)                                                                                                                                                              \\
                                                                                                                                                                                                                                                                                   & \multirow{2}{*}{Gamification (direct: OECD,  Luguri, Gray)}                                                                                                                                                 & Pay-to-Play (direct: FTC)                                                                                                                                                                                  \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Grinding (direct: FTC)                                                                                                                                                                                     \\
                                                                                                                                                                                                                                                                                   & Attention Capture                                                                                                                                                                                         &                                                                                                                                                                                                            \\
\midrule
\multirow{9}{*}{Social Engineering}                                                                                                                                                                                                                                                & \multirow{2}{*}{Scarcity and Popularity Claims (direct: Mathur, Luguri, FTC,  CMA)}                                                                                                                          & Auto-Play (direct: FTC)                                                                                                                                                                                    \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & High Demand (direct: Luguri, EUCOM, OECD, FTC, Mathur)                                                                                                                                                         \\
                                                                                                                                                                                                                                                                                   & \multirow{3}{*}{Social Proof (direct:Mathur, Luguri, EUCOM, OECD)}                                                                                                                                           & Low Stock (direct: FTC, EUCOM, Luguri, OECD, Mathur)                                                                                                                                                           \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Endorsements and Testimonials (direct: Luguri, OECD, Mathur, FTC, EUCOM; indirect: FTC (deceptive consumer testmonials))                                                                                       \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Parasocial Pressure (inferred: FTC (parasocial relationship pressure + deceptive celebrity endorsements))                                                                                                  \\
                                                                                                                                                                                                                                                                                   & \multirow{2}{*}{Urgency (direct: Luguri, Mathur, EUCOM, FTC, OECD)}                                                                                                                                           & Activity Messages (direct: Luguri, Mathur, EUCOM, FTC, OECD)                                                                                                                                                   \\
                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                           & Countdown Timer (direct:Mathur, FTC, OECD, EUCOM, Luguri)                                                                                                                                                      \\
                                                                                                                                                                                                                                                                                   & Shaming                                                                                                                                                                                                   & Limited Time Message (direct: Mathur, Luguri, EUCOM, OECD, FTC)                                                                                                                                                \\
                                                                                                                                                                                                                                                                                   & Personalization (direct: CMA)                                                                                                                                                                             & Confirmshaming (direct:OECD, Mathur, Brignull, Luguri, FTC, EUCOM)                                                                                                                                             
\end{tabularx}
\end{table*}

==> todo.tex <==
\section{To Do List}

\begin{itemize}
    \item Section Items

    \begin{enumerate}
        \item @Cris to include in the discussion section the legal parag
        \item @Cris to include DP harms related to cases
        \item Create \textit{Motivation and Background} section to provide a narrative that introduces the reader to dark patterns work in its current form (e.g., SIG, regulatory action, HCI interest) and its history in practitioner lit.
        \item Polish \textit{Methodology} to include justification for selection of sources + indication of how we extended ontology mapping to definitional work. \textbf{CMG Drafted}
        \item Update \textit{Introduction} once the motivation is set and clarify/finalize contributions.
        \item Add historical background to \textit{Mapping the Evolution...} to include Harry's evolution of types, the progression of academic mappings, etc.
        \item Draft the \textit{Creating a Definitional Structure} introduction and decide on how to introduce the definition forms, examples of definitions (or all of them?; or does a complete list only go in the appendix?), and elements of definitions. \textbf{CMG need to finish off low-level definitions and draft this section, but should be pretty straightforward}
        \item Draft the \textit{Extending the Ontology} to include mapping (subsumption or extension) from two existing contemporary sources. This includes both the mapping itself and the logic so others could do similar work on their own in future to extend the ontology. \textbf{CMG: perhaps using an example from the Hidaka paper for straightforward mapping + Thomas' patterns to show a more complex mapping is enough?}
        \item Enrich and update \textit{Discussion}. \textbf{CMG: needs to be a focus on the "structure for transdisciplinary action" part of the title}
        \item Draft the \textit{Implications and Future Work} to include clear ways for the ontology to be built upon in multiple sectors.
    \end{enumerate}
    
    \item \textbf{Figures}
    \begin{enumerate}
        \item Update ontology figure to include corrected mappings from airtable. \textbf{(CMG TO DO)}
        \item Create timeline with progression of dark patterns sources used in this paper? (TM) (CMG probably not needed anymore)
        \item Create evolution of darkpatterns.org types to show progression of the initial set of pattern types. \textbf{(CMG DONE)}
        \item Create a visual depiction of our method \textbf{(CMG DONE)}
        \item Create version of Miro mapping of dark patterns types in the HCI literature. (CMG) OR an example drawn from this instead. (TM) \textbf{CMG Added the Miro playground as figure}
    \end{enumerate}
\end{itemize}

\iffalse
\subsection{Connecting enforcement sanctions to multiple levels of patterns and combinations of pattern types.}
\CS{moved to section 7.1}

%By mapping case law to the ontology, this ontology may be used to support regulatory and enforcement measures  by indicating where dark patterns practices at multiple levels and in multiple combinations are at play, and are deemed to be illegal. %or improper. 

Dark patterns have been observed to be a recurrent phenomenon in regulatory cases by enforcers (Data Protection Authorities 'DPAs' and Consumer protection authorities) under relevant laws for more than a decade, though few cases explicitly designate them as such. Decisions analyse several practices that are related to dark patterns, but without qualifying each practice into a concrete granular type of dark pattern. Thus, concrete dark patterns type or categories are not mentioned in case law.
%
By mapping case law to the ontology, regulators can gain additional knowledge % and support i
 identifying where dark patterns practices at multiple levels and in multiple combinations are at play, and are deemed to be illegal per jurisdiction~\cite{Leiser-2022-regpluralismGDPR/UCPD}. 
%
Current descriptions of the use of dark patterns often report infringements only at a general level of abstraction\footnote{Cristiana Santos, Arianna Rossi, The emergence of dark patterns as a legal concept in case law, Internet Policy Review, available at \url{https://policyreview.info/articles/news/emergence-of-dark-patterns-as-a-legal-concept}} %lowest level (often re-using Brignull's original pattern types) 
and in doing so, could miss lower granularity
%broader abstractions
that may translate across domains. 
%
Connecting caselaw to multiple levels of dark patterns has the potential to inform enforcers of different legislative instruments in the EU/US and reduce the risks of gaps or overlaps. 
For instance, the Italian Data Protection Authority has already added the keyword “dark pattern” to the available tags of their online database\footnote{\url{https://www.garanteprivacy.it/temi/internet-e-nuove-tecnologie/dark-pattern}} - a useful effort that should be extended to official and unofficial searchable databases of enforcers’ decisions.
%
%
Early enforcement actions in relation to subscription services and online tracking (a focus in both EU and FTC enforcement) has started to reveal the interplay of multiple pattern types at multiple levels in causing user confusion, manipulation, or coercion, and other broad genres of manipulation that might benefit from similar characterizations.
%\CS{in our current work of case law and dark patterns we understand that certain practices look common in both consumer law cases and in data protection cases; e.g. the practices of "Misled into registering/ Difficulty in carrying out the booking process without purchasing said service", or "Unknowingly subscription after free registration and trial period" (that look like cases of  Privacy Zuckering and forced action) look like data protection practices of storing cookies in the users device before consent or after the user withdraw consent (forced action and sneaking?). this means that it is important to have a higher level types (meso) that regulators can make use of, which can then be substantiated into more granular practices at domain level}
%\CS{mapping dp to sanctions could help in monitoring and auditability for compliance. We can maybe cite some examples}
%\CS{we can give you a list of case law practices that correlate with DP for us to support this argument from different domains, not only data prot}
\fi
